A Proof of the CSP Dichotomy Conjecture

Many natural combinatorial problems can be expressed as constraint satisfaction problems. This class of problems is known to be NP-complete in general, but certain restrictions on the form of the constraints can ensure tractability. The standard way to parameterize interesting subclasses of the constraint satisfaction problem is via finite constraint languages. The main problem is to classify those subclasses that are solvable in polynomial time and those that are NP-complete. It was conjectured that if a constraint language has a weak near unanimity polymorphism then the corresponding constraint satisfaction problem is tractable, otherwise it is NP-complete. In the paper we present an algorithm that solves Constraint Satisfaction Problem in polynomial time for constraint languages having a weak near unanimity polymorphism, which proves the remaining part of the conjecture.

==> Crap.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckIrreducibility}{$\Theta$}
    \For{$k=1,\ldots,n$}
        \For{$\sigma_{k}$ is a maximal congruence on $D_{k}$}
            \State{$I:=\{k\}$}
            \For{$C\in\Theta$, $i\in I$, $j\notin I$ such that $x_{i}$ and $x_{j}$ are in the scope of $C$}
                \State{$\delta:=\proj_{x_{i},x_{j}} C$}
                \State{$\sigma_{j}(x,y) := \exists x'\exists y' \delta(x',x)\wedge \delta(y',y)\wedge \sigma_{i}(x',y')$}
                \If{$\sigma_{j}$ is a proper equivalence relation}
                    \State{$I:=I\cup\{j\}$}
                \EndIf
            \EndFor
            \For{$i\in I$}
                \State{$D_{i}':=\varnothing$}
                \For{$a\in D_{i}$}
                    \For{$j\in I$}
                        \State{$E_{j}:=\FindClass(a,i,j)$}
%                        \Comment{Choose an equivalence class of $D_{j}$ corresponding to                         $a\in D_{i}$} 
                    \EndFor
                    \State{$\mathbf{X'} = \{x_{i}\mid i\in I\}$}                        
                    \If{$\Solve(\Reduce(\proj_{X'}\Theta,
                        x_{i}\in\{a\},x_{j}\in E_{j} \text{for} j\neq i))  = \mbox{``Solution"}$}
                        \State{$D_{i}':=D_{i}'\cup\{a\}$}
                    \EndIf
                \EndFor
                \If{$D_{i}'=\varnothing$}
                    \Return{``No solution"}
                \ElsIf{$D_{i}'\neq D_{i}$} 
                    \Return{$(x_{i},D_{i}')$} 
                \EndIf
            \EndFor
        \EndFor
    \EndFor
    \Return{\mbox{``Ok"}}
\EndFunction
\end{algorithmic}
\end{algorithm}












\begin{THMParPropertyForSubcontraint}
Suppose $D^{(0)},\ldots,D^{(s)}$ is a minimal strategy for a cycle-consistent irreducible CSP instance
$\Theta$,
$\Upsilon(x_{1},\ldots,x_{n})$ is a subconstraint of $\Theta$,
the solution set of $\Upsilon^{(s)}$ is subdirect,
$k\in\{1,2,\dots,n-1\}$,
$\Var(\Upsilon) = \{x_{1},\ldots,x_{n},u_{1},\ldots,u_{t}\}$,
$$\Omega =
\Upsilon_{x_{1},\ldots,x_{k},u_{1},\ldots,u_{t}}^{y_{1},\ldots,y_{k},v_{1},\ldots,v_{t}}
\wedge
\Upsilon_{x_{k+1},\ldots,x_{n},u_{1},\ldots,u_{t}}^{y_{k+1},\ldots,y_{n},v_{t+1},\ldots,v_{2t}}
\wedge
\Upsilon_{x_{1},\ldots,x_{n},u_{1},\ldots,u_{t}}^{y_{1},\ldots,y_{n},v_{2t+1},\ldots,v_{3t}},$$
and $\Theta^{(s)}$ has no solutions.
Then $(\Theta\setminus\Upsilon)\cup\Omega$ has no solutions in $D^{(s)}$.
\end{THMParPropertyForSubcontraint}

\begin{proof}
Put $\Theta' = (\Theta\setminus\Upsilon)\cup\Omega$.
Since $\Omega$ is a covering of $\Upsilon$, 
Lemma~\ref{ExpandedConsistencyLemma} implies that 
$\Theta\cup\Omega$ is cycle-consistent and irreducible.
Assume that $\Theta'$ has a solution in $D^{(s)}$.

Assume that $|D^{(s)}_{x}|=1$ for every variable $x$ of $\Theta$. Since the reduction $D^{(s)}$ is 1-consistent,
we get a solution, which contradicts the fact that
$\Theta$ has no solutions in $D^{(s)}$.

If we have a nontrivial binary absorption, or a nontrivial center, or a nontrivial PC subuniverse on some domain $D_{x}^{(s)}$, then
by Theorems~\ref{NextReductionOne},~\ref{NextReductionTwo},
there exists a minimal nonlinear reduction $D^{(s+1)}$ for $\Theta$.
As we explained before, $\size(D^{(s+1)})<\size(D^{(s)})$.
This reduction can be naturally expanded on $\Theta'$.
By Lemma~\ref{ProperReductionPreservesCycleConAndIrreducability},
$\Theta'^{(s)}$ is cycle-consistent and irreducible.
By the inductive assumption for Theorem~\ref{CannotLooseSolution},
$\Theta'$ has a solution in $D^{(s+1)}$.
This contradicts the inductive assumption.

It remains to consider the case when $\ConLin(D_{x}^{(s)})$ is proper for every $x$ such that $|D_{x}^{(s)}|>1$.
Let $\alpha$ be a solution of $\Theta'$ in $D^{(s)}$.
Let the projection of $\alpha$ onto the variables $x_{1},\ldots,x_n$ be $(a_{1},\ldots,a_{n})$.

Assume that $\rho$ does not have the parallelogram property.
Without loss of generality we can assume that there exist $c_{1},\ldots,c_{n}$
and $d_{1},\ldots,d_{n}$
such that
\begin{align*}
(c_{1},\ldots,c_{k},c_{k+1},\ldots,c_{n})&\notin\rho,\\
(c_{1},\ldots,c_{k},d_{k+1},\ldots,d_{n})&\in\rho,\\
(d_{1},\ldots,d_{k},c_{k+1},\ldots,c_{n})&\in\rho,\\
(d_{1},\ldots,d_{k},d_{k+1},\ldots,d_{n})&\in\rho.
\end{align*}
Put
\begin{align*}
\rho'(x_{1},\ldots,x_{n}) =
\exists y_{1}\dots\exists y_{n}\;
\rho(x_{1},\ldots,x_{k},y_{k+1},\ldots,y_{n})
\wedge&\\
\rho(y_{1},\ldots,y_{k},x_{k+1},\ldots,x_{n})
\wedge
\rho(y_{1},\ldots,y_{k},y_{k+1},\ldots,y_{n}).
\end{align*}
Obviously, $\rho\subsetneq\rho'$
%$(c_{1},\ldots,c_{n})\in\rho'\setminus \rho$
and $\rho'\in\Gamma$,
therefore $(a_{1},\ldots,a_{n})\in\rho'.$
Hence, there exist $b_{1},\ldots,b_{n}$ such that
\begin{align*}
(a_{1},\ldots,a_{k},b_{k+1},\ldots,b_{n})&\in\rho,\\
(b_{1},\ldots,b_{k},a_{k+1},\ldots,a_{n})&\in\rho,\\
(b_{1},\ldots,b_{k},b_{k+1},\ldots,b_{n})&\in\rho.
\end{align*}
By Lemma~\ref{ParProperty},
there exists a tuple
$(e_{1},\ldots,e_{n})\in \rho$
such that
$(a_{i},e_{i})\in\LinCon(D_{x_{i}}^{(s)})$  for every $i$.

Consider the minimal linear reduction $D^{(s+1)}$ of 
$\Theta^{(s)}$ such that 
$\alpha\in D^{(s+1)}$.
Then $(e_{1},\ldots,e_{n})\in \rho^{(s+1)}$,
and by Lemma~\ref{ProperReductionPreservesSubdirectness},
$D^{(s+1)}$ is a 1-consistent reduction of $\Theta^{(s)}$.
Since $\Theta'$ has a solution in $D^{(s+1)}$,
$\rho(x_{1},\ldots,x_{n})$ is crucial in $D^{(s+1)}$.
We get a longer minimal strategy with smaller $\size(D^{(s+1)})$, hence by the inductive assumption
the relation $\rho$ is a critical relation with the parallelogram property.




We recursively build a strategy
$D^{(s)},D^{(s+1)},\ldots,D^{(q)}$
for $\Theta\cup\Omega = \Theta'\cup\Upsilon$ 
satisfying the following conditions:
\begin{enumerate}
    \item 
    $D^{(s)},D^{(s+1)},\dots,D^{(q)}$ is a minimal strategy for $\Theta'^{(s)}$;
    \item if $s\le j<q$ and $D^{(j+1)}$ is a linear reduction, then for each $i\in\{1,2,\dots,t\}$
    $$D_{u_{i}}^{(j+1)} = 
    \proj_{n+i}(\rho'\cap 
    (D_{x_{1}}^{(j+1)}\times\dots\times D_{x_{n}}^{(j+1)}
    \times
    D_{u_{1}}^{(j)}\times\dots\times D_{u_{t}}^{(j)})),
    $$
    where $\rho'$ is the relation defined by 
    $\Upsilon(x_{1},\ldots,x_{n},u_1,\ldots,u_t)$;
\item the solution set of $\Upsilon^{(j)}$ is subdirect for $s\le j\le q$;
\item $\Theta'$ has a solution in $D^{(q)}$.
\end{enumerate}

Note that here we allow 
$D^{(j)}$ to be equal to $D^{(j+1)}$ in a strategy, which can happen 
if $D^{(j+1)}$ is a proper reduction for 
$\Upsilon^{(j)}$ but not proper for $\Theta'^{(j)}$.


We will prove that we can make this sequence longer while
$|D^{(q)}_{x_{i}}|>1$ for some $i$.
%Assume that $|D^{(q)}_{x_{i}}|>1$ for some $i$.
By Theorem~\ref{NextReduction}, 
there exists a nontrivial one-of-four subuniverse on 
$D^{(q)}_{x}$ if $|D^{(q)}_{x}|>1$.
We consider two cases:

Case 1. Suppose there exists a nontrivial binary absorption, or a nontrivial center, or a nontrivial PC congruence on some domain $D_{x}^{(q)}$. 
Then applying Theorems~\ref{NextReductionOne}, \ref{NextReductionTwo}
to the strategy 
$D^{(0)},D^{(1)},\dots,D^{(q)}$ of $\Theta\cup\Omega$, 
we conclude that there exists a minimal 1-consistent nonlinear reduction $D^{(q+1)}$
for $(\Theta\cup\Omega)^{(q)}$.
By Lemma~\ref{ProperReductionPreservesCycleConAndIrreducability},
$\Theta'^{(q)}$ and  
$\Upsilon^{(q)}$ are cycle-consistent and irreducible.
By Theorem~\ref{CannotLooseSolution}
$\Theta'$ has a solution in $D^{(q+1)}$
and
$\Upsilon$ has a solution in $D^{(q+1)}$.
By Lemma~\ref{ProperReductionPreservesSubdirectness},
the solution set of $\Upsilon^{(q+1)}$ is subdirect.
%By Lemma~\ref{ProperReductionPreservesSubdirectness},
%$\Upsilon^{(s+1)}(x_{1},\ldots,x_{n})$ is subdirect.
%By the inductive assumption, we get a contradiction with the fact that $\Theta'^{(q+1)}$ has no solutions.
%Thus, $\Theta^{(s+1)}$ has no solutions, $\Theta'^{(s+1)}$ has a solution, which
%contradicts the inductive assumption.
Thus, we made the sequence longer.

Case 2. $\ConLin(D_{x}^{(q)})$ is proper for every $x$ such that $|D_{x}^{(q)}|>1$.
%%%%Without loss of generality we can assume that there exist $a_{1},\ldots,a_{n},b_{1},\ldots,b_{n}$ such that
%%%%\begin{align*}
%%%%(a_{1},\ldots,a_{k},a_{k+1},\ldots,a_{n})&\notin\rho,\\
%%%%(a_{1},\ldots,a_{k},b_{k+1},\ldots,b_{n})&\in\rho,\\
%%%%(b_{1},\ldots,b_{k},a_{k+1},\ldots,a_{n})&\in\rho,\\
%%%%(b_{1},\ldots,b_{k},b_{k+1},\ldots,b_{n})&\in\rho.
%%%%\end{align*}
%%%%Put
%%%%$$\Upsilon'= \Upsilon(y_{1},\ldots,y_{k},x_{k+1},\ldots,x_{n})\wedge
%%%%\Upsilon(x_{1},\ldots,x_{k},y_{k+1},\ldots,y_{n})\wedge
%%%%\Upsilon(y_{1},\ldots,y_{k},y_{k+1},\ldots,y_{n}).$$
%%%%By $\Theta'$ we denote the instance obtained from $\Theta$ by replacement of $\Upsilon$ by $\Upsilon'$.
%%%%Since $\Upsilon'^{(v)}(x_{1},\ldots,x_{n})$ is weaker
%%%%than $\Upsilon^{(v)}(x_{1},\ldots,x_{n})$,
%%%%$\Theta'$ has a solution in $D^{(s)}$.
%Let $\Upsilon^{(s)}(x_{1},\ldots,x_{n})$ define the relation $\rho$.
Let $\alpha$ be a solution of $\Theta'$ in $D^{(q)}$.
We define the new linear reduction 
$D^{(q+1)}$ as follows.
For all variables 
but $u_{1},\ldots,u_{t}$,
we choose an equivalence class
of $\ConLin(D_{x}^{(q)})$
containing the corresponding element of 
the solution $\alpha$.
For the variable $u_{i}$ we define 
$D_{u_{i}}^{(q+1)}$ by the formula in (2) 
from the above list for $j=q$.
By Lemma~\ref{ProperReductionPreservesSubdirectness},
$D^{(q+1)}$ is  
1-consistent for $\Theta'$.
Note that it does not follow from the definition 
that 
$D_{u_{i}}^{(q+1)}$ is not empty and we will prove this later.

Let the projection of $\alpha$ onto the variables $x_{1},\ldots,x_n$ be $(a_{1},\ldots,a_{n})$.
Suppose $\Upsilon^{(s)}(x_{1},\ldots,x_{n})$ defines a relation $\rho$.
Since $\alpha$ is a solution of $\Theta'^{(s)}$, there exist
$b_{1},\ldots,b_{n}$ such that
\begin{align*}
(a_{1},\ldots,a_{k},b_{k+1},\ldots,b_{n})&\in\rho,\\
(b_{1},\ldots,b_{k},a_{k+1},\ldots,a_{n})&\in\rho,\\
(b_{1},\ldots,b_{k},b_{k+1},\ldots,b_{n})&\in\rho.
\end{align*}

%By Lemma~\ref{ProperReductionPreservesSubdirectness},
%$D^{(s)},\ldots,D^{(q)}$ is a minimal strategy for $\rho$.
By Lemma~\ref{ParProperty},
there exists a tuple
$(d_{1},\ldots,d_{n})\in \rho$
such that
$(a_{i},d_{i})\in\LinCon(D_{x_{i}}^{(q)})$ for every $i$.
Therefore, $(\Upsilon^{(s)}(x_{1},\ldots,x_{n}))^{(q+1)}$ is not empty.

Let us show by induction on $j=s,s+1,\dots,q$ that $(\Upsilon^{(j)}(x_{1},\ldots,x_{n}))^{(q+1)}$ is not empty. For $j=s$ we already know this.
If the reduction $D^{(j+1)}$ is not linear, then 
Theorem~\ref{PreviousReductions}
implies that 
if 
$(\Upsilon^{(j)}(x_{1},\ldots,x_{n}))^{(q+1)}$
is not empty
then $(\Upsilon^{(j+1)}(x_{1},\ldots,x_{n}))^{(q+1)}$
is not empty.
If the reduction $D^{(j+1)}$ is linear then it follows from the definition of $D_{u_i}^{(j+1)}$
that $(\Upsilon^{(j+1)}(x_{1},\ldots,x_{n}))^{(q+1)}$ is not empty.
Thus, we can prove that $(\Upsilon^{(q)}(x_{1},\ldots,x_{n}))^{(q+1)}$ is not empty, 
and therefore $D_{u_i}^{(q+1)}$ is not empty
for every $i$. 
Considering the solution set of $\Upsilon$ and 
applying Corollary~\ref{LinearImplies}, 
we derive that 
$D_{u_{i}}^{(q+1)}$ is a linear subuniverse of 
$D_{u_{i}}^{(q)}$. Hence,
the reduction $D^{(q+1)}$ is a 1-consistent linear reduction
for $\Upsilon^{(q)}$.

By Lemma~\ref{ProperReductionPreservesSubdirectness},
$(\Upsilon^{(q)}(x_{1},\ldots,x_{n}))^{(q+1)}$
is subdirect. 
From the definition of 
$D_{u_{i}}^{(q+1)}$ 
we derive that 
the projection of
the solution set of $\Upsilon^{(q+1)}$ onto 
$u_{i}$ is $D_{u_{i}}^{(q+1)}$ 
for every $i$, which means that 
the solution set of $\Upsilon^{(q+1)}$
is subdirect.
Hence, we get a longer strategy having all the necessary properties.

Thus, we showed that we can make the sequence longer 
until  $|D^{(q)}_{x_{i}}|=1$ for every $i$.
Assume that we reached this final state.
Since both $\Upsilon$ and $\Theta'$ has a solution in $D^{(q)}$
and $x_{1},\dots,x_{n}$ are 
its only common variables,
$\Theta$ has a solution in $D^{(q)}$,
which contradicts the fact that
$\Theta$ has no solutions in~$D^{(s)}$.
\end{proof}



==> GreatFacts.tex <==
\begin{lem}\label{FactorByStableCongruence}
Suppose 
$\sigma$ is a congruence on $D$, 
$B$ is one-of-four subuniverse of $D$ stable under $\sigma$.
Then 
$\{b/\sigma\mid b\in B\}$ is a one-of-four subuniverse of $D/\sigma$ of the same type as $B$.
\end{lem}
\begin{proof}
For a binary subuniverse and a center it follows from 
Corollaries~\ref{AbsorptionQuotient} and \ref{CenterQuotient},
respectively.
Suppose $B$ is a linear subuniverse.
Let $\delta$ be the minimal congruence containing both 
$\sigma$ and $\ConLin(D)$.
By Lemma~\ref{LinearAlgebrasAreClosed}, 
$D/\delta$ is a linear algebra.
Since $B$ is stable under $\delta$, 
$\{b/\sigma\mid b\in B\}$ is a linear subuniverse of $D/\sigma$.

It remains to consider the case when 
$B$ is a PC subuniverse of $D$, that is, 
$B=E_{1}\cap \dots \cap E_{s}$, where 
$E_{i}$ is an equivalence class of 
a PC congruence $\sigma_{i}$ for every $i$.
Let $\delta$ be the minimal congruence containing 
$\sigma$ and $\sigma_{1}\cap\dots\cap\sigma_{s}$.
By Lemma~\ref{BiggerThanPC}, 
$\delta$ is an intersection of 
PC congruences 
$\delta_{1},\ldots,\delta_{t}$.
Since $B$ is stable under $\delta$
and $B$ is an equivalence class
of $\sigma_{1}\cap\dots\cap\sigma_{s}$,
$B$ is an equivalence class of $\delta$.
Hence, 
$\{b/\sigma\mid b\in B\}$ is an intersection of equivalence 
classes of congruences on $D/\sigma$ corresponding to 
$\delta_{1},\dots,\delta_{t}$.
\end{proof}


==> PCB.tex <==
\subsection{Additional}

IMPORTANT! Sometimes we use $\Theta(x_{1},\dots,x_{n})$ to denote the relation.

A subuniverse $A'$ of $\mathbf A$ is called \emph{a PC subuniverse}
if $A' = E_{1}\cap\dots\cap E_{s}$,
where $E_{i}$ is an equivalence class of a congruence $\sigma_{i}$ such that $\mathbf A/\sigma_{i}$ is a PC algebra {\bf without binary absorption or center}.

$B\subseteq A$ is called \emph{a one-of-four subuniverse}
if it is a binary absorbing subuniverse, 
a center, a linear subuniverse, or a PC subuniverse. 
We say that $B$ is a one-of-four subuniverse of \emph{absorbing type}, 
\emph{central type}, \emph{linear type}, or \emph{PC type}.





==> Psueducode.tex <==
\section{Appendix}

\newpage
\begin{algorithm}
\begin{algorithmic}[1]
\Function{\Solve}{$\Theta$}
  \State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}
\Repeat
  \State{$\Output := \AnswerOrReduce(\Theta)$}
  \If{$\Output = \mbox{``Solution"}$} \Return{``Solution"}
  \EndIf
  \If{$\Output = \mbox{``No solution"}$} \Return{``No solution"}
  \EndIf
  \If{$\Output = (x_i,U)$} \Comment{$\varnothing \ne U\subset D_i$}
    \State{$\Theta:= \Reduce(\Theta,(D_1,\dots,D_{i-1},U,D_{i+1},\dots,D_{n}))$}
    \Comment{Set $D_{i}=U$}
     %\State{$D_i:=U$}
     %\State{update $\calC$}
  \EndIf
\Until{Done}
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{AnswerOrReduce}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}

  \State{$\Output := \CheckCycleConsistency(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf
    \If{$|D_{i}|=1$ for every $i$}
        \Return{``Solution"}
    \EndIf
  \State{$\Output := \CheckIrreducibility(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf
  
  \State{$\Output := \CheckWeakerInstance(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf

  \If{$B_{i}$ is a binary absorbing subuniverse of $D_{i}$}  \Return{$(x_{i},B_{i})$}
  \EndIf

\If{$C_{i}$ is a center of $D_{i}$}  \Return{$(x_{i},C_{i})$}
  \EndIf
  
\If{$\sigma$ is a congruence on $D_{i}$ and $(D_{i};w)/\sigma$ is polynomially complete} 

Choose an equivalence class $E$ of $\sigma$ 

\Return{$(x_{i},E)$}
\EndIf
\Return{$\SolveLinearCase(\Theta)$}

\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{SolveLinearCase}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}

\State{$\Theta_{L} := \FactorizeInstance(\Theta)$}
\State{$Eq := \varnothing$} \Comment{The equations we add to $\Theta_{L}$}
\Repeat
  \State{$\phi := \SolveLinearSystem(\Theta_{L}\cup Eq)$}
  
  \Comment{$\phi(\mathbb Z_{q_{1}}\times\dots\times\mathbb Z_{q_{k}})$ is the solution set of $\Theta_{L}\cup Eq$}
  \If{$\phi  = \varnothing$}  
    \Return{``No solution"}
  \EndIf    
    \If{$\Solve(\Reduce(\Theta, \phi(0,0,\ldots,0)))  = \mbox{``Solution"}$}
    \Return{``Solution"}
    \ElsIf{k=0} 
        \Return{``No solution"} \Comment{$\Theta_{L}$ has just one solution}
    \EndIf

\State{$\Theta':= \RemoveTriv(\Theta)$}
\Repeat \Comment{Try to weaken $\Theta'$}
    \State{$\Changed:= false$}
    \For{$C\in \Theta'$} 
        \State{$\Omega:= \RemoveTriv(\WeakenConstraint(\Theta',C))$}
        \If{$\neg\CheckAllTuples(\Omega,\phi)$}
            \State{$\Theta':=\Omega$}
            \State{$\Changed:= true$}
            \Break
        \EndIf
    \EndFor
\Until{$\neg\Changed$} \Comment{$\Theta'$ cannot be weakened anymore}
  \If{$\Theta'$ is not linked} 
    \State{$Eq := Eq\cup\FindEquationsForNonlinked(\Theta')$}
  \Else 
  \State{$Eq := Eq\cup\{\FindOneEquationLinked(\Theta',\phi)\}$}
\EndIf
\Until{Done}
\EndFunction
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckAllTuples}{$\Theta$, $\phi$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a linear system of equations $\phi$}
    \If{$\Solve(\Reduce(\Theta,\phi(0,\ldots,0))) = \mbox{``No solution"}$}
        \Return{$false$}
    \EndIf
   \For{$i=1,2,\ldots,k$}
        \State{$t := (\underbrace{0,\ldots,0,1}_{i},0,\ldots,0)$}
        \If{$\Solve(\Reduce(\Theta,\phi(t))) = \mbox{``No solution"}$}
            \Return{$false$}
        \EndIf
    \EndFor
    \Return {$true$};
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{\FindOneEquationLinked}{$\Theta,\phi$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a system of linear equations $\phi$}
    \State{$t := \varnothing$}     \Comment{We search for a tuple $t$ outside of the solution set}    
    \If{$\Solve(\Reduce(\Theta,\phi(0,\ldots,0))) = \mbox{``No solution"}$}
        \State{$t:= (0,\ldots,0)$}
    \Else
        \For{$i=1,2,\ldots,k$}
            \State{$t' := (\underbrace{0,\ldots,0,1}_{i},0,\ldots,0)$}
            \If{$\Solve(\Reduce(\Theta,\phi(t'))) = \mbox{``No solution"}$}
                \State{$t := t'$}
                \Break
            \EndIf
        \EndFor
    \EndIf
    \If{$t = \varnothing$} \Return{``$0=0$''} 
    \EndIf
    \For{$i=1,2,\ldots,k$}
        \State{$b_{i}:=0$}
        \For{$a\in \mathbb Z_{j_{i}}\setminus\{t(i)\}$}
            \State{$t' := t$}
            \State{$t'(i):= a$}
            \If{$\Solve(\Reduce(\Theta,\phi(t'))) = \mbox{``Solution"}$}         \State{$b_{i} := 1/(a-t(i))$}
            \EndIf
        \EndFor
    \EndFor    
    \Return {``$b_{1}(y_{1}-t(1)) +\dots + b_{k}(y_{k}-t(k)) = 1$''}
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\FindEquationsForNonlinked}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$}
%    \State{Let $\psi$ be a natural bijection from $\mathbb Z_{j_{1}}\times \dots \times \mathbb Z_{j_{s}}\to L_{1}\times\dots\times L_{n}$}   
    \State{$I := \{1\}$}     \Comment{$I$ is the set of independent variables}
    \State{$E := \varnothing$}     \Comment{We start with an empty set of equations}    
   \For{$j=1,2,\ldots,r$}
    \State{$e := \FindOneEquationNonlinked(\Theta,I\cup\{j\})$}     %\Comment{Something about the equations}
    \If{$e = \mbox{``$0=0$"}$}  \Comment{$j$-th variable is independent}
        \State{$I := I\cup \{j\}$}
    \ElsIf{$e = \mbox{``$0=1$"}$}
        \Return{$\mbox{``No solution"}$}
    \Else
        \State{$E := E\cup e$}     \Comment{Add the equation we found}    
    \EndIf
    \EndFor
    \Return {$E$}
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\FindOneEquationNonlinked}{$\Theta,I$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, 
$I = \{i_1,\ldots,i_{h}\}$ a set of variables}
    \State{$t := \varnothing$}     \Comment{We search for a tuple $t$ outside of the solution set}            
    \If{$\neg\CheckTuple(\Theta,I,(0,\ldots,0))$} 
        \State{$t:= (0,\ldots,0)$}
    \Else
        \For{$j=1,2,\ldots,h$}
            \State{$t' := (\underbrace{0,\ldots,0,1}_{j},0,\ldots,0)$}
            \If{$\neg\CheckTuple(\Theta,I,t')$} 
                \State{$t := t'$}
                \Break
            \EndIf
        \EndFor
    \EndIf
    \If{$t = \varnothing$} \Return{``$0=0$''} 
    \EndIf
    \For{$j=1,2,\ldots,h$}
        \State{$b_{j}:=0$}
        \For{$a\in \mathbb Z_{p_{i_{j}}}\setminus\{t(j)\}$}
            \State{$t' := t$}
            \State{$t'(j):= a$}
            \If{$\CheckTuple(\Theta,I,t')$} 
                \State{$b_{j} := 1/(a-t(j))$}
            \EndIf
        \EndFor
    \EndFor    
    \Return {``$b_{1}(z_{i_{1}}-t(1)) +\dots + b_{h}(z_{i_{h}}-t(r)) = 1$''}
%    \Return {``$\Sum_{i\in I} b_{i}(z_{i}-t()) +\dots + b_{r}(z_{r}-t(r)) = 1$''}    
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckTuple}{$\Theta,I,t$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, 
$I$ a subset of variables, $t$ a tuple of length $|I|$}
    \State{$R:=\{\alpha\in \mathbb Z_{p_{1}}\times\dots\times\mathbb Z_{p_{r}} \mid \proj_{I}(\alpha) = t\}$}    
    \Comment{We don't really calculate $R$}
    \For{$i=1,2,\ldots,n$}
        \State{$D_{i}':=\bigcup_{E\in\proj_{i}(\psi(R))} E$} \Comment{We calculate $D_{i}'$}
    \EndFor
    \If{$\SolveNonlinked(\Reduce(\Theta,(D_{1}',\dots,D_{n}')) = \mbox{``Solution''}$}
        \Return true
    \Else 
        ~\Return false
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckCycleConsistency}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$}
    \For{$i,j\in\{1,2,\ldots,n\}$} 
    \Comment{Calculate binary projections $\rho_{i,j}$}
        \State{$\rho_{i,j} := D_{i}\times D_{j}$}
        \For{$C\in\Theta$}        
            \State{$\rho_{i,j} :=\rho_{i,j}\cap \proj_{x_i,x_j} C$}
            \Comment{$\proj_{x_i,x_j} C$ is the projection 
            of $C$ onto $x_{i},x_{j}$}
        \EndFor
    \EndFor
    \Repeat \Comment{Propagate constraints to reduce  $\rho_{i,j}$}
        \State{$\Changed:= false$}
        \For{$i,j,k\in\{1,2,\ldots,n\}$} 
            \State{$\rho_{i,j}'(x,y) := \exists z\;
            \rho_{i,j}(x,y)\wedge \rho_{i,k}(x,z)\wedge 
            \rho_{k,j}(z,y)$}
            \If{$\rho_{i,j} \neq \rho_{i,j}'$}
                \State{$\rho_{i,j}:=\rho_{i,j}'$}
                \State{$\Changed:= true$}               
            \EndIf
        \EndFor
    \Until{$\neg\Changed$} \Comment{We cannot reduce $\rho_{i,j}$ anymore}
    \For{$i,j\in\{1,2,\ldots,n\}$} 
        \If{$\rho_{i,j}=\varnothing$}
            \Return{``No solution"}
        \EndIf
        \If{$\proj_{1}(\rho_{i,j})\neq D_{i}$}
            \Return{$(x_{i},\proj_{1}(\rho_{i,j}))$}
        \EndIf
        \If{$\proj_{2}(\rho_{i,j})\neq D_{j}$}
            \Return{$(x_{j},\proj_{2}(\rho_{i,j}))$}
        \EndIf

    \EndFor
    \Return{\mbox{``Ok"}}
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckIrreducibility}{$\Theta$}
    \For{$k=1,\ldots,n$}
        \For{$\sigma_{k}=\{E_{k}^{1},\ldots,E_{k}^{t}\}$ is a maximal congruence on $D_{k}$}
            \State{$I:=\{k\}$}
            \Repeat
                \State{$\Changed:=false$}
                \For{$C\in\Theta$, $i\in I$, $j\notin I$ such that $x_{i}$ and $x_{j}$ are in the scope of $C$}
                    \State{$\delta:=\proj_{x_{i},x_{j}} C$} 
                    \Comment{$\proj_{x_{i},x_{j}} C$ is a projection of $C$ onto $x_{i},x_{j}$}
%                \State{$\sigma_{j}(x,y) := \exists x'\exists y' \delta(x',x)\wedge \delta(y',y)\wedge 
%\sigma_{i}(x',y')$}                    
                    \For{$u=1,2,\dots,t$}  
                        \Comment{Calculate partition on $D_{j}$}
                            \State{$E_{j}^{u}:= \{a\in D_{j}\mid \exists b\in E_{i}^{u}: (a,b)\in \delta\}$}
                    \EndFor                    
                    \If{$E_{j}^{1},\dots,E_{j}^{t}$ are disjoint}
                        \State{$I:=I\cup\{j\}$}
                        \State{$\Changed:=true$}
                        \Break
                    \EndIf
                \EndFor
            \Until{$\neg\Changed$}
            \For{$i\in I$}
                \State{$D_{i}':=\varnothing$}
                \For{$a\in D_{i}$}
                    \State{Choose $u$ such that $a\in E_{i}^{u}$}
%                    \For{$j\in I$}
%                        \State{$E_{j}:=\FindClass(a,i,j)$}
%                        \Comment{Choose an equivalence class of $D_{j}$ corresponding to                         $a\in D_{i}$} 
%                    \EndFor
                    \For{$j=1,2,\ldots,n$}
                        \If{$j=i$}
                            \State{$E_{j} := \{a\}$}
                        \ElsIf{$j\in I$}
                            \State{$E_{j} := E_{j}^{u}$}
                        \Else
                            \State{$E_{j} := D_{j}$}
                        \EndIf                        
                    \EndFor
                    \State{$\mathbf{X'} = \{x_{i}\mid i\in I\}$}                        
                    \If{$\Solve(\proj_{\mathbf{X'}}(\Reduce(\Theta,(E_{1},\ldots,E_{n}))))  = \mbox{``Solution"}$}
                        \State{$D_{i}':=D_{i}'\cup\{a\}$}
                    \EndIf
                \EndFor
                \If{$D_{i}'=\varnothing$}
                    \Return{``No solution"}
                \ElsIf{$D_{i}'\neq D_{i}$} 
                    \Return{$(x_{i},D_{i}')$} 
                \EndIf
            \EndFor
        \EndFor
    \EndFor
    \Return{\mbox{``Ok"}}
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckWeakerInstance}{$\Theta$}
  \State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$}
    \State{$\Theta'= \WeakenEveryConstraint(\Theta)$}
    \For{$i=1,\ldots,n$}
        \State{$D_{i}'=\varnothing$}
        \For{$a\in D_{i}$}
            \State{$\Output := \Solve(\Reduce(\Theta,D_{1},\dots,D_{i-1},
            \{a\},D_{i+1},\dots,D_{n}))$}
            \If{$\Output = \mbox{``Solution"}$}
                \State{$D_{i}':=D_{i}'\cup \{a\}$}
            \EndIf
        \EndFor
        \If{$D_{i}'=\varnothing$}
            \Return{``No solution"}
        \ElsIf{$D_{i}'\neq D_{i}$} 
            \Return{$(x_{i},D_{i}')$} 
        \EndIf
    \EndFor
    \Return{``No solution"}    
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\SolveNonlinked}{$\Theta$}
  \State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$}
    \State{$\Theta':=\proj_{\mathbf{X'}}(\Theta)$}
    \Comment{Remove variables that never occur}
%    $\Theta'=(\mathbf{X'},\mahtbf{D'},\mahtbf{C'})$,
%$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$
%    \Comment{$\Theta'$ is the projection onto all variables from the scope of a constraint of $\Theta$}    
    \For{a linked component $(D_{1}',\dots,D_{n'}')$ of $\Theta'$} 
%    \Comment{We recursively solve every linked component}
%        \State{$\Output := \Solve(\Reduce(\Theta,D_{1}',\dots,D_{n}'))$}
%        \If{$\Output = \mbox{``Solution"}$}
        \If{$\Solve(\Reduce(\Theta',(D_{1}',\dots,D_{n'}'))) = \mbox{``Solution"}$}
            \Return{``Solution"}
        \EndIf
    \EndFor
    \Return{``No solution"}    
\EndFunction
\end{algorithmic}
\end{algorithm}



\newpage


\begin{thm}\label{NextReduction}
Suppose $\mathbf{A} = (A;w)$ is an algebra, $w$ is a special WNU of arity $m$.
Then one of the following conditions hold
\begin{enumerate}
\item there exists a nontrivial binary absorbing subuniverse $B\subsetneq A$,
\item there exists a nontrivial center $C\subsetneq A$,
\item there exists a proper congruence $\sigma$ on $A$ such that
$(A;w)/\sigma$ is polynomially complete,
\item there exists a proper congruence $\sigma$ on $A$ such that
$(A;w)/\sigma$ is isomorphic to $(\mathbb Z_{p};x_{1}+\dots +x_{m})$.
\end{enumerate}
\end{thm}


\begin{thm}\label{AbsorptionCenterStep}
Suppose $\Theta$ is a cycle-consistent irreducible CSP instance,
$B$ is a binary absorbing set or a center of $D_{i}$.
Then $\Theta$ has a solution if and only if
$\Theta$ has a solution with $x_{i}\in B$.
\end{thm}


%%\begin{thm}\label{CenterStep}
%%Suppose $\Theta$ is a cycle-consistent irreducible CSP instance,
%%$C$ is a center of $D_{i}$.
%%Then $\Theta$ has a solution if and only if
%%$\Theta$ has a solution with $x_{i}\in C$.
%%\end{thm}

\begin{thm}\label{PCStepThm}
Suppose $\Theta$ is a cycle-consistent irreducible CSP instance,
there does not exist a binary absorbing subuniverse or a center on $D_{j}$
for every $j$,
$(D_{i};w)/\sigma$ is a polynomially complete algebra, % for a congruence $\sigma$,
$E$ is an equivalence class of $\sigma$.
Then $\Theta$ has a solution if and only if
$\Theta$ has a solution with $x_{i}\in E$.
\end{thm}



%Let $p$ be a prime number,
%$\delta_{i}$ be a minimal congruence on $D_{i}$ such that
%$(D_{i};w)/\delta_{i}$ is isomorphic to
%$(\mathbb Z_{p}^{j};x_{1}+\dots+x_{m})$
%for some $j\ge 0$.

%%We denote $D_{i}/\delta_{i}$ by $L_{i}$.
%%We define a new CSP instance $\Theta_{L}$ with domains $L_{1},\ldots,L_{n}$.
%%To every constraint $((x_{i_1},\ldots,x_{i_s});\rho)\in \Theta$
%%we assign a constraint
%%$((x_{i_1}',\ldots,x_{i_s}');\rho')$,
%%where $\rho'\subseteq L_{i_{1}}\times\dots\times L_{i_{s}}$
%%and $$(E_{1},\ldots,E_{s})\in\rho'\Leftrightarrow
%%(E_{1}\times\dots\times E_{s})\cap\rho\neq\varnothing.$$
%%The constraints of $\Theta_{L}$ are all constraints that are assigned to constraints of $\Theta$.
%%
%%\begin{thm}\label{LinearStep}
%%Suppose $\Theta$ is a cycle-consistent irreducible linked CSP instance,
%%$(D_{1}',\ldots,D_{n}')$ is a solution of $\Theta_{L}$,
%%$\Theta$ is crucial in $(D_{1}',\ldots,D_{n}')$,
%%there does not exist a binary absorbing subuniverse or a center on $D_{j}$
%%for every $j$.
%%Then there exists a constraint $((x_{i_1},\ldots,x_{i_s}),\rho)$ in $\Theta$
%%and a subuniverse $\sigma$ of ${D_{i_1}}\times\dots\times {D_{i_s}}\times {\mathbb Z_{p}}$
%%such that
%%the projection of $\sigma$ onto the first $s$ coordinates
%%is bigger than $\rho$ but
%%the projection of $\sigma\cap (D_{i_1}\times\dots\times D_{i_s}\times \{0\})$
%%onto the first $s$ coordinates is equal to $\rho$.
%%\end{thm}






\begin{thm}\label{LinearStep}
Suppose the following conditions hold:
\begin{enumerate}
\item $\Theta$ is a linked cycle-consistent irreducible CSP instance with domain set
$(D_{1},\ldots,D_{n})$;
\item there does not exist a nontrivial binary absorbing subuniverse or a nontrivial center on $D_{j}$ for every $j$;
\item if we replace every constraint of $\Theta$ by all weaker constraints then the obtained instance
has a solution with $x_{i} = b$ for every $i$ and $b\in D_{i}$;
%\item $\Theta_{L}$ is $\Theta$ factorized by the minimal linear congruences, 
%the domains of the variables of $\Theta_{L}$ are $L_{1},\ldots,L_{n}$;
\item $L_{i} = D_{i}/\sigma_{i}$ for every $i$, where $\sigma_{i}$ is the minimal linear congruence on $D_{i}$;
\item $\phi:\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}}
\to L_{1}\times\dots\times L_{n}$;
\item if we replace any constraint of 
$\Theta$ by all weaker constraint then for every $(a_{1},\ldots,a_{k})\in \mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}}$ 
there exists a solution of the new instance in 
$\phi(a_{1},\ldots,a_{k})$.
%\item $B= \{(a_{1},\dots,a_{k})\mid \Theta \text{ has a solution in }\phi(a_1,\dots,a_{k})\}$
\end{enumerate}
Then 
$\{(a_{1},\dots,a_{k})\mid \Theta \text{ has a solution in }\phi(a_1,\dots,a_{k})\}$ is 
either empty, or is full, or is an affine subspace of codimension 1 (the solution set of a single linear equation).
\end{thm}


%\subsection{Correctness of the algorithm}

%In this section we will prove that the algorithm 
%actually solves the constraint satisfaction problem.

%As it was mentioned before, 



==> algorithm.tex <==
\section{Algorithm}\label{Algorithm}
\subsection{Main part}\label{AlgorithmMainPart}


Suppose we have a constraint language $\Gamma_{0}$ that is preserved by an idempotent WNU operation.
As it was mentioned before,
$\Gamma_{0}$ is also preserved by a special WNU operation $w$.
Let $k_{0}$ be the maximal arity of the relations in $\Gamma_{0}$.
By $\Gamma$ we denote the set of all relations of arity at most $k_{0}$
that are preserved by $w$.
Obviously, $\Gamma_{0}\subseteq \Gamma$, therefore $\CSP(\Gamma_{0})$ can be reduced to $\CSP(\Gamma)$

In this section we provide an algorithm that solves $\CSP(\Gamma)$ in polynomial time.
Suppose we have a CSP instance $\Theta = \langle \mathbf{X} , \mathbf{D} , \mathbf{C} \rangle$,
where
$\mathbf{X}=\{x_1,\ldots ,x_n\}$ is a set of variables,
$\mathbf{D}=\{D_{1},\ldots ,D_{n}\}$ is a set of the respective domains,
$\mathbf{C}=\{C_{1},\ldots ,C_{q}\}$ is a set of constraints.
Let the arity of the WNU $w$ be equal to $m$.

The algorithm is recursive, the list of all possible recursive calls is given in the end of this subsection.
One of the main recursive calls is the reduction of a subuniverse $D_{i}$ to $D_{i}'$
such that either $\Theta$ has a solution with $x_{i}\in D_{i}'$,
or it has no solutions at all.
%%
%%The algorithm returns one of the following results:
%%\begin{itemize}
%%\item It returns a subuniverse $D_{i}'\subsetneq D_{i}$ such that
%%either $\Theta$ has a solution with $x_{i}\in D_{i}'$,
%%or it has no solutions at all;
%%\item It returns ``no solutions'';
%%\item It returns ``there exists a solution''.
%%\end{itemize}

%It is easy to see that if the algorithm is polynomial,
%it can be used to solve $\CSP(\Gamma)$ in polynomial time.

\begin{step}\label{CycleConsistencyStep}
Check whether $\Theta$ is cycle-consistent. If not then we reduce a domain $D_{i}$ for some $i$
or state that there are no solutions.
%If we reduce $D_{i}$ to $\varnothing$, then $\Theta$ has no solutions.
\end{step}

%%Note that a CSP instance is called \emph{irreducible} if
%%for any subinstance $\Theta'$ and any set of
%%variables $X'$ the projection of $\Theta'$ onto $X'$ is either
%%linked, or subdirect.

\begin{step}\label{IrreducibilityStep}
Check whether $\Theta$ is irreducible.  If not then we reduce a domain $D_{i}$ for some $i$
or state that there are no solutions.
%If we reduce $D_{i}$ to $\varnothing$, then $\Theta$ has no solutions.
\end{step}

\begin{step}\label{FullSimplificationStep}
Replace every constraint of $\Theta$ by all weaker constraints.
Recursively calling the algorithm, check that the obtained instance has a solution
with $x_{i}=b$ for every $i\in\{1,2,\ldots,n\}$ and $b\in D_{i}$.
If not, reduce $D_{i}$ to the projection onto $x_{i}$ of the solution set of the obtained instance.
%%
%%Replace every constraint of $\Theta$ by all weaker constraints. Check that the obtained instance has a solution
%%with $x_{i}=b$ for every $i\in\{1,2,\ldots,n\}$ and $b\in D_{i}$.
%%If not reduce $D_{i}$ to the projection onto $x_{i}$ of the solution set of the obtained instance.
\end{step}

By Theorem~\ref{AbsorptionCenterStep} we cannot loose the only solution while doing the following two steps.
\begin{step}\label{AbsorptionStep}
If $D_{i}$ has a binary absorbing subuniverse $B_{i}\subsetneq D_{i}$ for some $i$, then we reduce $D_{i}$ to $B_{i}$.
\end{step}

\begin{step}\label{CenterStep}
If $D_{i}$ has a center $C_{i}\subsetneq D_{i}$  for some $i$, then we reduce $D_{i}$ to $C_{i}$.
\end{step}

By Theorem~\ref{PCStepThm} we can do the following step.
\begin{step}\label{PCStep}
If there exists a congruence $\sigma$ on $D_{i}$ such that
the algebra $(D_{i};w)/\sigma$ is polynomially complete, then we reduce $D_{i}$ to
any equivalence class of $\sigma$.
\end{step}

By Theorem~\ref{NextReduction},
it remains to consider the case when
for every domain $D_{i}$
there exists a congruence $\sigma_{i}$ on $D_{i}$
such that
$(D_{i};w)/\sigma_{i}$ is linear, i.e. it is isomorphic to
$(\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}};x_{1}+\dots+x_{m})$
for prime numbers $p_{1},\ldots,p_{l}$.
Moreover, $\sigma_{i}$ is proper if $|D_{i}|>1$.
%To simplify explanation, we are going to handle one prime number $p_{i}$ in one step.
%Note that it is possible to handle all prime numbers simultaneously, which is probably more efficient.

%\begin{step}
%Choose a prime number $p$ such that there exist $i$ and a congruence $\delta$ on $D_{i}$
%for which $(D_{i};w)/\delta$ is isomorphic to $(\mathbb Z_{p};x_{1}+\dots+x_{m})$.
%\end{step}

%Choose a prime number $p$ that appears in the list of prime numbers mentioned above.
%For every $i$ by
%$\delta_{i}$ we denote the minimal congruence on $D_{i}$
%such that
%$(D_{i};w)/\delta_{i}$ is isomorphic to
%$(\mathbb Z_{p}^{j};x_{1}+\dots+x_{m})$
%for some $j\ge 0$.
We denote $D_{i}/\sigma_{i}$ by $L_{i}$.
We define a new CSP instance $\Theta_{L}$ with domains $L_{1},\ldots,L_{n}$.
To every constraint $((x_{i_1},\ldots,x_{i_s});\rho)\in \Theta$
we assign a constraint
$((x_{i_1}',\ldots,x_{i_s}');\rho')$,
where $\rho'\subseteq L_{i_{1}}\times\dots\times L_{i_{s}}$
and $(E_{1},\ldots,E_{s})\in\rho'\Leftrightarrow
(E_{1}\times\dots\times E_{s})\cap\rho\neq\varnothing.$
The constraints of $\Theta_{L}$ are all constraints that are assigned to the constraints of $\Theta$.


%Since every $(L_{i};w)$  is isomorphic to
%$(\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}};x_{1}+\ldots+x_{m})$
%for some prime numbers $p_{1},\ldots,p_{l}$ and  some $j$,
%and
Since every relation on $\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}}$ preserved by $x_{1}+\ldots+x_{m}$ is known to be
a conjunction of linear equations,
the instance $\Theta_{L}$ can be viewed as a system of linear equations
in $\mathbb Z_{p}$ for different $p$.
%To simplify the explanation we include variables with different domains in one equation.
Note that all essential variables of every equation have the same domain.
%only variables with domain $\mathbb Z_{p}$ for a fixed $p$ are not dummy in this equation.
%a field (probably several systems of equations in different fields).

Our general idea is to add some linear equations to $\Theta_{L}$ so that
for any solution of $\Theta_{L}$ there exists the corresponding solution of $\Theta$.
We start with the empty set of equations $Eq$, which is
a set of constraints on $L_{1},\ldots,L_{n}$.
%Let $Eq$ be a set of constraints on $L_{1},\ldots,L_{n}$ (which are linear equations).
%We start with an empty set.

\begin{step}
Put $Eq:=\varnothing$.
\end{step}

\begin{step}\label{AddingEquationCycle}
Solve the system of linear equations $\Theta_{L}\cup Eq$
and choose independent variables
$y_{1},\ldots,y_{k}$.
If it has no solutions then $\Theta$ has no solutions.
If it has just one solution, then, recursively calling the algorithm, solve the reduction of $\Theta$ to this solution.
Either we get a solution of $\Theta$, or $\Theta$ has no solutions.
\end{step}
%If it has just one solution, then solve the reduction of $\Theta$ to this solution.
%If we don't get a solution to $\Theta$, then $\Theta$ has no solutions.


Then there exist
${Z} = \mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}}$ and
a linear mapping $\phi\colon Z \to L_{1}\times\dots\times L_{n}$
such that any solution of $\Theta_{L}\cup Eq$ can be obtained
as $\phi(a_{1},\ldots,a_{k})$ for some $(a_{1},\ldots,a_{k})\in {Z}$.

Note that for any tuple $(a_{1},\ldots,a_{k})\in {Z}$
we can check recursively whether $\Theta$ has a solution
in $\phi(a_{1},\ldots,a_{k})$.
To do this, we just need to solve an easier CSP instance (on smaller domains).
Similarly, we can check whether $\Theta$ has a solution in
$\phi(a_{1},\ldots,a_{k})$
for every $(a_{1},\ldots,a_{k})\in \mathbb {Z}$.
To do this, we just need to check the
existence of a solution in $\phi(0,\ldots,0,1,0,\ldots,0)$ and
$\phi(0,\ldots,0)$  for any position of $1$.


\begin{step}\label{SolveZeros}
Check whether $\Theta$ has a solution in $\phi(0,\ldots,0)$. If it has then stop the algorithm.
\end{step}


\begin{step}
Put $\Theta':= \Theta$. Iteratively remove from $\Theta'$ all
constraints that are weaker than some other constraints of $\Theta'$.
\end{step}
\begin{step}\label{SimplificationCycle}
For every constraint $C\in\Theta'$
\begin{enumerate}
\item Let $\Omega$ be obtained from $\Theta'$ by replacing the constraint $C\in\Theta'$ by all weaker constraints without
dummy variables. Remove from $\Omega$ all constraints that are weaker than some other constraints of $\Omega$.
%Denote the obtained instance by $\Omega$.
%\item Replace a constraint $C\in\Theta'$ by all bigger constraints.
%Denote the obtained instance by $\Omega$.
%to get an instance $\Omega$.
\item If $\Omega$ has no solutions in
$\phi(a_{1},\ldots,a_{k})$
for some $(a_{1},\ldots,a_{k})\in {Z}$,
then put $\Theta':=\Omega$. Repeat Step~\ref{SimplificationCycle}.
\end{enumerate}
\end{step}

At this moment, the CSP instance $\Theta'$ has the following property.
$\Theta'$ has no solutions in $\phi(b_{1},\ldots,b_{k})$
for some $(b_{1},\ldots,b_{k})\in {Z}$,
but if we replace any constraint $C\in\Theta'$ by all weaker constraints,
then we get an instance that has a solution
in $\phi(a_{1},\ldots,a_{k})$
for every $(a_{1},\ldots,a_{k})\in {Z}$.
Therefore, %if we remove all non-maximal constraints, then
$\Theta'$ is crucial in
$\phi(b_{1},\ldots,b_{k})$.

%%%In the remaining steps we will find a new linear equation that can be added to the instance.
%%%These steps are based on the following idea.
%%%Suppose we have a linear equation in $\mathbb Z_{p}^{h}$ such that $(c_{1},c_{2},\ldots,c_{h})$ does not satisfy the equation.
%%%To find this equation
%%%it is sufficient to check
%%%for every $a$ and every $i$
%%%whether the tuple $(c_{1},\ldots,c_{i-1},a,c_{i+1},\ldots,c_{h})$ satisfies this equation.
%%%This means that to compute the equation
%%%it is sufficient to check at most $p\cdot h+1$ tuples: the first $(h+1)$ tuples to find a tuple that does not satisfy the equation,
%%%the next $(p-1)\cdot h$ tuples to find the equation.

In the remaining steps we will find a new linear equation that can be added to $\Theta_{L}$.
Suppose $V$ is an affine subspace of $\mathbb Z_{p}^{h}$ of dimension $h-1$, thus $V$ is the solution set of a linear equation
$c_1x_1 + \dots + c_h x_h = c_{0}$. Then the coefficients $c_0,c_{1},\dots,c_{h}$ can be learned (up to a multiplicative constant) by $(p\cdot h+1)$ queries of the form ``$(a_1,\ldots,a_h) \in V$?'' as follows.
First, we need at most $(h+1)$ queries to find a tuple $(d_{1},\ldots,d_{h})\notin V$. % that does not satisfy the equation.
Then, to find this equation it is sufficient to check for every $a$ and every $i$
whether the tuple $(d_{1},\ldots,d_{i-1},a,d_{i+1},\ldots,d_{h})$ satisfies this equation.



%%
%%Then we factorize every constraint to get
%%a CSP instance $\Omega_{L}$ on domains $L_{1},\ldots,L_{n},Z_{p}$.
%%We know that the projection of
%%the solution set of $\Omega_{L}$ onto
%%the first $n$ variables is a full relation.
%%Therefore, the solution set can be defined by one linear equation with the variable $z$.
%%Hence, the solution set of


\begin{step}\label{nonLinkedStep}
Suppose $\Theta'$ is not linked. For each $i$ from $1$ to $k$
\begin{enumerate}
\item Check that for every $(a_{1},\ldots,a_{i})\in \mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{i}}$
there exist $(a_{i+1},\ldots,a_{k})\in \mathbb Z_{q_{i+1}}\times \dots \times \mathbb Z_{q_{k}}$ and  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item If yes, go to the next $i$.
\item If no, then find an equation
$c_{1}y_{1}+\dots+c_{i}y_{i}=c_{0}$ such that
for every $(a_{1},\ldots,a_{i})\in
\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{i}}$
satisfying $c_{1}a_{1}+\dots+c_{i}a_{i}=c_{0}$
there exist $(a_{i+1},\ldots,a_{k})\in \mathbb Z_{q_{i+1}}\times \dots \times \mathbb Z_{q_{k}}$ and  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item Add the equation $c_{1}y_{1}+\dots+c_{i}y_{i}=c_{0}$ to Eq.
\item Go to Step~\ref{AddingEquationCycle}.
\end{enumerate}
\end{step}

If $\Theta'$ is linked, then by Theorem~\ref{LinearStep} there exists a constraint
$((x_{i_1},\ldots,x_{i_s}),\rho)$ in $\Theta'$
and a subuniverse $\sigma$ of $\mathbf{D_{i_1}}\times\dots\times \mathbf{D_{i_s}}\times \mathbf{\mathbb Z_{p}}$
such that
the projection of $\sigma$ onto the first $s$ coordinates
is bigger than $\rho$ but
the projection of $\sigma\cap (D_{i_1}\times\dots\times D_{i_s}\times \{0\})$
onto the first $s$ coordinates is equal to $\rho$.
Then we add a new variable $z$ with domain $\mathbb Z_{p}$
and replace
$((x_{i_1},\ldots,x_{i_s}),\rho)$ by
$((x_{i_1},\ldots,x_{i_s},z),\sigma)$.
We denote the obtained instance by $\Upsilon$.
Let
$L$ be the set of all tuples $(a_{1},\ldots,a_{k},b)\in
\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}} \times \mathbb Z_{p}$
such that $\Upsilon$ has a solution with $z=b$ in $\phi(a_{1},\ldots,a_{k})$.
We know that the projection of $L$ onto
the first $n$ coordinates is a full relation.
Therefore $L$ is defined by one linear equation.
If this equation is $z = b$ for some $b\neq 0$, then
both $\Theta'$ and $\Theta$ have no solutions.
Otherwise, we put $z=0$ in this equation and get
an equation that describes all $(a_{1},\ldots,a_{k})$ such that
$\Theta'$ has a solution in $\phi(a_{1},\ldots,a_{k})$.
It remains to find this equation.

\begin{step}\label{LinkedStep}
Suppose $\Theta'$ is linked.
\begin{enumerate}
\item Find
an equation
$c_{1}y_{1}+\dots+c_{k}y_{k} = c_{0}$
such that
for every $(a_{1},\ldots,a_{k})\in
(\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}})$
satisfying $c_{1}a_{1}+\dots+c_{k}a_{k}=c_{0}$
there exists  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item If the equation was not found then $\Theta$ has no solutions.
\item Add the equation $c_{1}a_{1}+\dots+c_{k}a_{k}=c_{0}$ to Eq.
\item Go to Step~\ref{AddingEquationCycle}.
\end{enumerate}
\end{step}


Note that every time we reduce our domains, we get constraint relations that are still from~$\Gamma$.

We have four types of recursive calls of the algorithm:
\begin{enumerate}
\item we reduce one domain $D_{i}$, for example to a binary absorbing subuniverse or to a center
(Steps \ref{CycleConsistencyStep}, \ref{AbsorptionStep}, \ref{CenterStep}, \ref{PCStep}).
\item we solve an instance that is not linked. In this case we divide the instance into the linked parts
and solve each of them independently
(Steps \ref{IrreducibilityStep}, \ref{nonLinkedStep}).
\item we replace every constraint by all weaker constraints and solve an easier CSP instance
(Step \ref{FullSimplificationStep}).
\item we reduce every domain $D_{i}$ such that
$|D_{i}|>1$
%$(D_{i};w)/\delta$ is isomorphic to
%$(\mathbb Z_{p};x_{1}+\dots+x_{m})$
%for some congruence $\delta$
(Steps \ref{AddingEquationCycle}, \ref{SolveZeros}, \ref{SimplificationCycle}, \ref{LinkedStep}).
\end{enumerate}
%%Either we just reduce one domain $D_{i}$, or
%%for a prime number $p$ we reduce all domains $D_{i}$ such that
%%$(D_{i};w)/\delta_{i}$ is isomorphic to
%%$(\mathbb Z_{p};x_{1}+\dots+x_{m})$
%%for some congruence $\delta_{i}$.


%While measuring the depth of the recursion, we do not consider recursive calls of type 1 and 3.
%With this assumption, Lemma~\ref{RecursionDepth} states that the recursion cannot be deeper than $|A|^{3}$.
Lemma~\ref{RecursionTwoDepth} states %and \ref{RecursionDepth} states that the depth
%of the recursive calls of type 2 and 4 is at most $|A|^{3}$,
the depth of the recursive calls of type 3 is at most $|\Gamma|$.
It is easy to see that the depth of the recursive calls of type 2 and 4 is at most $|A|$.


\subsection{Remaining parts}\label{AlgorithmRemaining}
In this section we explain Steps 1, 2, and 12 of the algorithm,
which were not clarified in the previous section.

\textbf{Provide cycle-consistency.}
To provide cycle-consistency it is sufficient to use constraint propagation providing (2,3)-consistency.
Formally, it can be done in the following way.
First, for every pair of variables $(x_{i},x_{j})$ we consider the
intersections of projections of all constraints onto these variables.
The corresponding relation we denote by $\rho_{i,j}$.
For every $i,j,k\in\{1,2,\ldots,n\}$
we replace
$\rho_{i,j}$ by $\rho_{i,j}'$
where $\rho_{i,j}'(x,y) = \exists  z \; \rho_{i,j}(x,y)\wedge \rho_{i,k}(x,z)\wedge \rho_{k,j}(z,y).$
It is not hard to see that this replacement does not change the solution set.

We repeat this procedure while we can change some $\rho_{i,j}$.
If at some moment we get a relation $\rho_{i,j}$ that is not subdirect in $D_{i}\times D_{j}$,
then we can either reduce $D_{i}$ or $D_{j}$, or,
 if $\rho_{i,j}$ is empty, state that there are no solutions.
If we cannot change any relation $\rho_{i,j}$ and every $\rho_{i,j}$ is subdirect in
$D_{i}\times D_{j}$, then the original CSP instance is cycle-consistent.

\textbf{Solve the instance that is not linked.}
Suppose the instance $\Theta$ is not linked and not fragmented, then it can be solved in the following way.
We say that an element $d_{i}\in D_{i}$
and an element $d_{j}\in D_{j}$ are \emph{linked}
if there exists a path that connects $d_{i}$ and $d_{j}$.
Let $P$ be the set of pairs $(i;a)$
such that $i\in\{1,2,\ldots,n\}$, $a\in D_{i}$.
Then $P$ can be divided into the linked components.

It is easy to see that it is sufficient to solve
the problem for
every linked component and join the results.
Precisely, for a linked component
by
$D_{i}'$ we denote the set of all elements $d$
such that
$(i,d)$ is in the component.
It is easy to see that $\varnothing\subsetneq D_{i}'\subsetneq D_{i}$ for every $i$.
Therefore, the reduction to $(D_{1}',\ldots,D_{n}')$ is a CSP instance on smaller domains.

\textbf{Check irreducibility.}
For every $k\in\{1,2,\ldots,n\}$ and every maximal
congruence $\sigma_{k}$ on $D_{k}$ we do the following.
\begin{enumerate}
\item Put $I = \{k\}$.
\item Choose a constraint $C$ having the variable $x_{i}$ in the scope for some $i\in I$, choose another variable $x_{j}$ from
the scope such that $j\notin I$.
\item Denote the projection of $C$ onto $(x_{i},x_{j})$ by $\delta$.
\item Put $\sigma_{j}(x,y) = \exists x'\exists y' \delta(x',x)\wedge \delta(y',y)\wedge \sigma_{i}(x',y')$.
If $\sigma_{j}$ is a proper equivalence relation,
then add $j$ to $I$.
\item go to the next $C$, $x_{i}$, and $x_{j}$ in 2.
\end{enumerate}
As a result we get a set $I$ and
a congruence $\sigma_{i}$ on $D_{i}$ for every $i\in I$.
Put $\mathbf{X'} = \{x_{i}\mid i\in I\}$.
It follows from the construction
that for every equivalence class $E_{k}$ of $\sigma_{k}$
and every $i\in I$
there exists a unique equivalence class $E_{i}$ of $\sigma_{i}$
such that there can be a solution with $x_{k}\in E_{k}$
and $x_{i}\in E_{i}$.
Thus, for every equivalence class of $\sigma_{k}$
we have a reduction to the instance on smaller domains.
Then for every $i$ and $a\in E_{i}$ we consider the corresponding reduction
and check whether there exists a solution with $x_{i} = a$.

Thus, we can check whether the solution set of the projection of the instance onto $\mathbf{X'}$ is subdirect or empty.
If it is empty then we state that there are no solutions.
If it is not subdirect, then we can reduce the corresponding domain.
If it is subdirect, then we
go to the next $k\in\{1,2,\ldots,n\}$ and next maximal
congruence $\sigma_{k}$ on $D_{k}$, and repeat the procedure.




==> algorithm_copy.tex <==
\newcommand{\Solve}{\mbox{\textsc{Solve}}}
\newcommand{\AnswerOrReduce}{\mbox{\textsc{AnswerOrReduce}}}
\newcommand{\CheckCycleConsistency}{\mbox{\textsc{CheckCycleConsistency}}}
\newcommand{\CheckIrreducibility}{\mbox{\textsc{CheckIrreducibility}}}
\newcommand{\CheckWeakerInstance}{\mbox{\textsc{CheckWeakerInstance}}}
\newcommand{\SolveLinearCase}{\mbox{\textsc{SolveLinearCase}}}
\newcommand{\RemoveTriv}{\mbox{\textsc{RemoveTrivialities}}}
\newcommand{\FactorizeInstance}{\mbox{\textsc{FactorizeInstance}}}
\newcommand{\Reduce}{\mbox{\textsc{Reduce}}}
\newcommand{\SolveLinearSystem}{\mbox{\textsc{SolveLinearSystem}}}
\newcommand{\WeakenConstraint}{\mbox{\textsc{WeakenConstraint}}}
\newcommand{\CheckAllTuples}{\mbox{\textsc{CheckAllTuples}}}
\newcommand{\SolveNonlinked}{\mbox{\textsc{SolveNonlinked}}}
\newcommand{\FindOneEquationLinked}{\mbox{\textsc{FindOneEquationLinked}}}
\newcommand{\FindOneEquationNonlinked}{\mbox{\textsc{FindOneEquationNonlinked}}}
\newcommand{\FindEquationsForNonlinked}{\mbox{\textsc{FindEquationsForNonlinked}}}
\newcommand{\CheckTuple}{\mbox{\textsc{CheckTuple}}}
\newcommand{\type}{\mbox{\textsc{type}}}

\newcommand{\Break}{\State \textbf{break} }

\newcommand{\Output}{\mbox{Output}}
\newcommand{\Changed}{\mbox{Changed}}
\newcommand{\calC}{\mathbf{C}}
\newcommand{\calD}{\mathbf{D}}
\newcommand{\X}{\mathbf{X}}

\section{Algorithm}\label{Algorithm}
\subsection{Main part}\label{AlgorithmMainPart}

Suppose we have a constraint language $\Gamma_{0}$ that is preserved by an idempotent WNU operation.
As it was mentioned before,
$\Gamma_{0}$ is also preserved by a special WNU operation $w$.
Let $k_{0}$ be the maximal arity of the relations in $\Gamma_{0}$.
By $\Gamma$ we denote the set of all relations of arity at most $k_{0}$
that are preserved by $w$.
Obviously, $\Gamma_{0}\subseteq \Gamma$, therefore $\CSP(\Gamma_{0})$ can be reduced to $\CSP(\Gamma)$

In this section we provide an algorithm that solves $\CSP(\Gamma)$ in polynomial time.
Suppose we have a CSP instance $\Theta = \langle \mathbf{X} , \mathbf{D} , \mathbf{C} \rangle$,
where
$\mathbf{X}=\{x_1,\ldots ,x_n\}$ is a set of variables,
$\mathbf{D}=\{D_{1},\ldots ,D_{n}\}$ is a set of the respective domains,
$\mathbf{C}=\{C_{1},\ldots ,C_{q}\}$ is a set of constraints.
Let the arity of the WNU $w$ be equal to $m$.

The main part of the algorithm (function \Solve)
is an iterative loop; in each pass through the loop, the algorithm calls a subroutine $\AnswerOrReduce$ whose
job is to find a reduction of a domain or to terminate with the final answer.
If the reduction was found then we apply the function 
$\Reduce$, which takes an instance $\Theta=(\X,\calD,\calC)$ and a domain set 
$\mathbf{D'} = (D_1',\ldots,D_{n}')$, and returns a new instance 
$(\X,\mathbf{D'},\mathbf{C'})$, where 
$\mathbf{C'}=\{\rho\cap (D_{i_{1}}'\times\dots D_{i_{s}})\mid
    ((x_{i_{1}},\dots,x_{i_{s}}),\rho)\in\calC\}$.



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\Solve}{$\Theta$}
  \State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}
\Repeat
  \State{$\Output := \AnswerOrReduce(\Theta)$}
  \If{$\Output = \mbox{``Solution"}$} \Return{``Solution"}
  \EndIf
  \If{$\Output = \mbox{``No solution"}$} \Return{``No solution"}
  \EndIf
  \If{$\Output = (x_i,U)$} \Comment{$\varnothing \ne U\subset D_i$}
    \State{$\Theta:= \Reduce(\Theta,(D_1,\dots,D_{i-1},U,D_{i+1},\dots,D_{n}))$}
    \Comment{Set $D_{i}=U$}
     %\State{$D_i:=U$}
     %\State{update $\calC$}
  \EndIf
\Until{Done}
\EndFunction
\end{algorithmic}
\end{algorithm}


%\begin{algorithm}
%\begin{algorithmic}[1]
%\Function{\Reduce}{$\Theta,\mathbf{D'}$}
%  \State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
%$\mathbf{D'} = (D_{1}',\dots,D_{n}')$}
%%\State{$\calD := (D_{1}',\dots,D_{n}')$}
%%((x_{i_{1}},\dots,x_{i_{s}}),\rho)
%    \State{$\mathbf{C'}=\{\rho\cap (D_{i_{1}}'\times\dots D_{i_{s}})\mid
%    ((x_{i_{1}},\dots,x_{i_{s}}),\rho)\in\calC\} $}        
%    
%\Return{$(\X,\mathbf{D'},\mathbf{C'})$}    
%\EndFunction
%\end{algorithmic}
%\end{algorithm}

The function \AnswerOrReduce checks different types of consistency such as cycle-consistency and irreducibility, and reduce a domain if the instance is not consistent. 
If it is consistent, then either it reduces a domain to a 
a proper strong subset, or 
it uses \SolveLinearCase to 
solve the remaining case.

%we know that 
%the instance can be written as a system of linear equations module some congruence. In the last case we use \SolveLinearCase that will be 
%described in the next subsection. 

First, the function \AnswerOrReduce 
checks whether $\Theta$ is cycle-consistent (function \CheckCycleConsistency). 
If it is not cycle-consistent then either some domain can be reduced, or the instance has no solutions. In both cases we break the function and return the result. If it is cycle consistent then we go on.

If the size of every domain is one it returns that solution was found.

Then we check whether the instance is irreducible (function \CheckIrreducibility).  
If it is not irreducible then we return the result, otherwise we go on.

\begin{algorithm}
\begin{algorithmic}[1]
\Function{AnswerOrReduce}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}

  \State{$\Output := \CheckCycleConsistency(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf
    \If{$|D_{i}|=1$ for every $i$}
        \Return{``Solution"}
    \EndIf
  \State{$\Output := \CheckIrreducibility(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf
  
  \State{$\Output := \CheckWeakerInstance(\Theta)$}
  \If{$\Output \neq \mbox{``Ok"}$} \Return{$\Output$}
  \EndIf

  \If{$B_{i}$ is a binary absorbing subuniverse of $D_{i}$}  \Return{$(x_{i},B_{i})$}
  \EndIf

\If{$C_{i}$ is a center of $D_{i}$}  \Return{$(x_{i},C_{i})$}
  \EndIf
  
\If{$\sigma$ is a congruence on $D_{i}$ and $(D_{i};w)/\sigma$ is polynomially complete} 

Choose an equivalence class $E$ of $\sigma$ 

\Return{$(x_{i},E)$}
\EndIf
\Return{$\SolveLinearCase(\Theta)$}

\EndFunction
\end{algorithmic}
\end{algorithm}

Then we check a different type of consistency (function \CheckWeakerInstance).
We make a copy of $\Theta$, and replace each constraint by all weaker constraints without dummy variables. Recursively calling the algorithm, check that the obtained instance has a solution
with $x_{i}=b$ for every $i\in\{1,2,\ldots,n\}$ and $b\in D_{i}$.
If not, reduce $D_{i}$ to the projection onto $x_{i}$ of the solution set of the obtained instance. Otherwise, go on.

By Theorem~\ref{AbsorptionCenterStep} we cannot loose all solutions 
when reduce a domain to a
nontrivial binary absorbing set or 
to a nontrivial center. 
Thus, if $D_{i}$ has a binary absorbing subuniverse $B_{i}\subsetneq D_{i}$ for some $i$, then we reduce $D_{i}$ to $B_{i}$,
Similarly, if $C_{i}$ has a center $C_{i}\subsetneq D_{i}$ for some $i$, then we reduce $D_{i}$ to $B_{i}$

By Theorem~\ref{PCStepThm} we cannot loose all solutions 
when reduce a domain to an equivalence class of 
congruence $\sigma$ such that $(D_{i};w)/\sigma$ is polynomially complete.
Thus, if such a congruence on $D_{i}$ exists, we reduce $D_{i}$ to
its equivalence class.

By Theorem~\ref{NextReduction},
it remains to consider the case when
for every domain $D_{i}$
there exists a congruence $\sigma_{i}$ on $D_{i}$
such that
$(D_{i};w)/\sigma_{i}$ is linear, i.e. it is isomorphic to
$(\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}};x_{1}+\dots+x_{m})$
for prime numbers $p_{1},\ldots,p_{l}$.
Moreover, $\sigma_{i}$ is proper if $|D_{i}|>1$.
In this case the problem is solved by function \SolveLinearCase that will be described in the next subsection. 
A detailed description and a pseudocode for the functions 
\CheckCycleConsistency, \CheckIrreducibility, and \CheckWeakerInstance
will be given in subsection \ref{AlgorithmTechnicalities}

\subsection{Linear case}\label{AlgorithmLinearCase}

In this subsection we define the function \SolveLinearCase (see pseudocode), 
which applied only if on every domain $D_{i}$
there exists a congruence $\sigma_{i}$ on $D_{i}$
such that
$(D_{i};w)/\sigma_{i}$ is linear, i.e. it is isomorphic to
$(\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}};x_{1}+\dots+x_{m})$
for prime numbers $p_{1},\ldots,p_{l}$.
Note that modulo these congruences the instance can be viewed as a system of linear equations in a field. 

We denote $D_{i}/\sigma_{i}$ by $L_{i}$.
We define a new CSP instance $\Theta_{L}$ with domains $L_{1},\ldots,L_{n}$.
To every constraint $((x_{i_1},\ldots,x_{i_s});\rho)\in \Theta$
we assign a constraint
$((x_{i_1}',\ldots,x_{i_s}');\rho')$,
where $\rho'\subseteq L_{i_{1}}\times\dots\times L_{i_{s}}$
and $(E_{1},\ldots,E_{s})\in\rho'\Leftrightarrow
(E_{1}\times\dots\times E_{s})\cap\rho\neq\varnothing.$
The constraints of $\Theta_{L}$ are all constraints that are assigned to the constraints of $\Theta$.
The function generating the instance $\Theta_{L}$ from $\Theta$ is called
\FactorizeInstance in pseudocode.


\begin{algorithm}
\begin{algorithmic}[1]
\Function{SolveLinearCase}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta=(\X,\calD,\calC)$,
$\X=(x_1,\ldots,x_n)$, $\calD = (D_1,\ldots,D_n)$}

\State{$\Theta_{L} := \FactorizeInstance(\Theta)$}
\State{$Eq := \varnothing$} \Comment{The equations we add to $\Theta$}
\Repeat
  \State{$\phi := \SolveLinearSystem(\Theta_{L}\cup Eq)$}
  
  \Comment{$\phi(\mathbb Z_{q_{1}}\times\dots\times\mathbb Z_{q_{k}})$ is the solution set of $\Theta_{L}\cup Eq$}
  \If{$\phi  = \varnothing$}  
    \Return{``No solution"}
  \EndIf    
    \If{$\Solve(\Reduce(\Theta, \phi(0,0,\ldots,0)))  = \mbox{``Solution"}$}
    \Return{``Solution"}
    \ElsIf{k=0} 
        \Return{``No solution"} \Comment{$\Theta_{L}$ has just one solution}
    \EndIf

\State{$\Theta':= \RemoveTriv(\Theta)$}
\Repeat \Comment{Try to weaken $\Theta'$}
    \State{$\Changed:= false$}
    \For{$C\in \Theta'$} 
        \State{$\Omega:= \WeakenConstraint(\Theta',C)$}
        \If{$\neg\CheckAllTuples(\Omega,\phi)$}
            \State{$\Theta':=\Omega$}
            \State{$\Changed:= true$}
            \Break
        \EndIf
    \EndFor
\Until{$\neg\Changed$} \Comment{$\Theta'$ cannot be weakened anymore}
  \If{$\Theta'$ is not linked} 
    \State{$Eq := Eq\cup\FindEquationsForNonlinked(\Theta')$}
  \Else 
  \State{$Eq := Eq\cup\{\FindOneEquation(\Theta',\phi)\}$}
\EndIf
\Until{Done}
\EndFunction
\end{algorithmic}
\end{algorithm}


Since every relation on $\mathbb Z_{p_{1}}\times \dots \times \mathbb Z_{p_{l}}$ preserved by $x_{1}+\ldots+x_{m}$ is known \cite{sassa} to be
a conjunction of linear equations,
the instance $\Theta_{L}$ can be viewed as a system of linear equations
in $\mathbb Z_{p}$ for different $p$, where all variables in 
any equation have the same domain.

As it was described in Section \ref{ZFourExample}, 
we consider the set $A$, which is the solution set of $\Theta$ factorized by the congruences $\sigma_{1},\ldots,\sigma_{n}$, 
and the set $B$, which is the solution set of $\Theta_{L}$.
We know that $A\subseteq B$ and we want to check whether $A$ is empty.
We iteratively add new equations to the set $\Theta_{L}$ maintaining the 
property that $A\subseteq B$, and therefore reduce the dimension of $B$.
We start with the empty set of equations $Eq$.

%Our general idea is to add a set $Eq$ of linear equations to $\Theta_{L}$ so that
%for any solution of $\Theta_{L}$ there exists the corresponding solution of $\Theta$. 
%While doing this, we have to maintain the condition that for any solution 
%of $\Theta$ there is a corresponding solution of $\Theta_{L}\cup Eq$.

Then we apply function $\SolveLinearSystem$ to solve the system of linear equations $\Theta_{L}\cup Eq$.
The general solution (the set $B$) can be written as a 
linear mapping $\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}}\to 
L_{1}\times\dots\times L_{n}$, where $k$ is the number of 
independent variables.
Denote ${Z} = \mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}}$,
then any solution of $\Theta_{L}\cup Eq$ can be obtained
as $\phi(a_{1},\ldots,a_{k})$ for some $(a_{1},\ldots,a_{k})\in {Z}$.

Note that for any tuple $(a_{1},\ldots,a_{k})\in {Z}$
we can check recursively whether $\Theta$ has a solution
in $\phi(a_{1},\ldots,a_{k})$ (i.e. whether 
$\phi(a_{1},\ldots,a_{k})\in A$).
To do this, we just need to 
reduce the domains to the solution (function \Reduce)
and solve an easier CSP instance (on smaller domains).
Similarly, we can check whether $\Theta$ has a solution in
$\phi(a_{1},\ldots,a_{k})$
for every $(a_{1},\ldots,a_{k})\in \mathbb {Z}$ (i.e. whether $A=B$).
Since $A$ and $B$ are subspaces, we just need to check the
existence of a solution in $\phi(0,\ldots,0,1,0,\ldots,0)$ and
$\phi(0,\ldots,0)$  for any position of $1$.
See the pseudocode of the function \CheckAllTuples for the last procedure.

\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckAllTuples}{$\Theta$, $\phi$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a linear system of equations $\phi$}
    \If{$\Solve(\Reduce(\Theta,\phi(0,\ldots,0))) = \mbox{``No solution"}$}
        \Return{$false$}
    \EndIf
   \For{$i=1,2,\ldots,k)$}
        \State{$t := (\underbrace{0,\ldots,0,1}_{i},0,\ldots,0)$}
        \If{$\Solve(\Reduce(\Theta,\phi(t))) = \mbox{``No solution"}$}
            \Return{$false$}
        \EndIf
    \EndFor
    \Return {$true$};
\EndFunction
\end{algorithmic}
\end{algorithm}

If the system has no solutions then $\Theta$ has no solutions and we are done.
Otherwise, we check whether there exists a solution 
of $\Theta$ corresponding to the solution $\phi(0,0,\ldots,0)$ of $\Theta_{L}\cup Eq$. If $k=0$, i.e. 
$\Theta_{L}\cup Eq$ has the only solution, then we denote this solution by $\phi(0,0,\ldots,0)$.
%Thus, we check whether $\phi(0,0,\ldots,0)\in A$.

If $\Theta$ has a solution in $\phi(0,\ldots,0)$, then it remains to return the result ``Solution''. 
Otherwise, if $k=0$ then return the result ``No solution''. 

At this point (line 10 of the pseudocode of the function 
$\SolveLinearCase$), we have the property that 
the set $B$ is of dimension at least 1, and $A\neq B$, 
i.e. there exists a solution of the system of linear equations 
without corresponding solution of $\Theta$.

Then we iteratively remove from $\Theta$ all
constraints that are weaker than some other constraints of $\Theta$, 
remove all constraints without non-dummy variables, 
and replace every constraint by its projection onto non-dummy variables.
This procedure we denote by the function $\RemoveTriv$.
In the pseudocode of the function 
$\SolveLinearCase$ the new instance we denote by $\Theta'$.

Then we try to make the constraints of $\Theta'$ weaker maintaining the property 
that $A'\neq B$, where $A'$ is that the solution set of $\Theta'$ factorized by 
the congruences $\sigma_{1},\ldots,\sigma_{n}$.
Thus, we choose a constraint $C$, replace it by all weaker constraints 
without dummy variables (function $\WeakenConstraint$), 
and check using the function $\CheckAllTuples$ whether 
$A' = B$. If not, then we replace $\Theta'$ by the new weaker instance.

If we cannot make any constraint weaker maintaining the property 
$A'\neq B$,  then the CSP instance $\Theta'$ has the following property.
$\Theta'$ has no solutions in $\phi(b_{1},\ldots,b_{k})$
for some $(b_{1},\ldots,b_{k})\in {Z}$,
but if we replace any constraint $C\in\Theta'$ by all weaker constraints,
then we get an instance that has a solution
in $\phi(a_{1},\ldots,a_{k})$
for every $(a_{1},\ldots,a_{k})\in {Z}$.
Therefore, 
$\Theta'$ is crucial in
$\phi(b_{1},\ldots,b_{k})$.

Then, in line 20 of the function $\SolveLinearCase$ we have two options.
If $\Theta'$ is not linked then using the function $\FindEquationsForNonlinked$ we calculate its solution set factorized by the congruences (the set $A'$). 
This solution set can be represented as a set of linear equations, 
which we add to $Eq$ and therefore we replace $B$ by $A'\cap B$. 
Thus, we made $B$ smaller and we still have the property $A\subseteq B$, 
since $A'$ is a solution set of the instance $\Theta'$ which is weaker than 
$\Theta$.

If $\Theta'$ is linked then by Lemma~\ref{CodimensionOne}
either $A' = \varnothing$, or 
the dimension of $A'$ is equal to the dimension of $B$ minus 1, 
which allows us to find a new linear equation by solving polynomially many instances on smaller domains. We calculate this new equation 
by the function $\FindOneEquation$, which will be defined in the next subsection 
as well as the function $\FindEquationsForNonlinked$. 
Note that the new equation can be ``$0=1$'' if $A'=\varnothing$.

After new equations found, we go back to line 6 of the function 
$\SolveLinearCase$ and solve a system of linear equations again.
Since every time we reduce the dimension of $B$ by at least one, 
the procedure will stop in at most $n$ steps.

\subsection{Finding linear equations}

In this subsection we define 
the functions 
$\FindOneEquationLinked$, $\FindOneEquationNonlinked$, and  $\FindEquationsForNonlinked$, which 
allow us to find $A'$ and therefore add new equations to $\Theta_{L}$.

First, we explain how 
the function $\FindOneEquationLinked$ works.
%to find one equation on 
%variables $x_{1},\ldots,x_{h}$ if we can check the 
%whether a tuple $(a_1,\ldots,a_h)$ satisfies the equation.
Suppose $V$ is an affine subspace of $\mathbb Z_{p}^{h}$ of dimension $h-1$, thus $V$ is the solution set of a linear equation
$c_1x_1 + \dots + c_h x_h = c_{0}$. Then the coefficients $c_0,c_{1},\dots,c_{h}$ can be learned (up to a multiplicative constant) by $(p\cdot h+1)$ queries of the form ``$(a_1,\ldots,a_h) \in V$?'' as follows.
First, we need at most $(h+1)$ queries to find a tuple $(d_{1},\ldots,d_{h})\notin V$. 
Then, to find this equation it is sufficient to check for every $a$ and every $i$
whether the tuple $(d_{1},\ldots,d_{i-1},a,d_{i+1},\ldots,d_{h})$ satisfies this equation.
This procedure is explained in the pseudocode of the function $\FindOneEquationLinked$, where the query is replaced by 
the reduction of all domains to the corresponding solution 
(the function $\Reduce$ and a recursive call of the main function 
$\Solve$


Note that the function $\FindOneEquation$ takes four parameters as an input: the instance $\Theta$, a mapping $\phi:
\mathbb Z_{j_{1}}\times\dots\times\mathbb Z_{j_{s}}\to 
L_{1}\times\dots\times L_{n}$, a subset $I\subseteq \{1,2,\ldots,s\}$, 
and the type of the instance $\Theta$, which is either ``Linked'' or
``Not linked''. 
The aim of the function is to find an equation 
with the variables 

All these parameters are used in the function $\CheckTuple$ (see , because we check the queries differently for linked and non-linked instances.




\begin{algorithm}
\begin{algorithmic}[1]
\Function{\FindOneEquationNonLinked}{$\Theta,\psi,I$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a linear system of equations $\phi$}
    \State{$t := \varnothing$}     \Comment{We search for a tuple $t$ outside of the solution set}            
    \If{$\neg\CheckTuple(\Theta,\psi,I,(0,\ldots,0))$} 
        \State{$t:= (0,\ldots,0)$}
    \Else
        \For{$i=1,2,\ldots,|I|)$}
            \State{$t' := (\underbrace{0,\ldots,0,1}_{i},0,\ldots,0)$}
            \If{$\neg\CheckTuple(\Theta,\phi,I,t')$} 
                \State{$t := t'$}
                \Break
            \EndIf
        \EndFor
    \EndIf
    \If{$t = \varnothing$} \Return{``$0=0$''} 
    \EndIf
    \For{$i=1,2,\ldots,|I|$}
        \State{$b_{i}:=0$}
        \For{$a\in Z_{j_{i}}\setminus\{t(i)\}$}
            \State{$t' := t$}
            \State{$t'(i):= a$}
            \If{$\CheckTuple(\Theta,\phi,I,t',\type)$} 
                \State{$b_{i} := 1/(a-t(i))$}
            \EndIf
        \EndFor
    \EndFor    
    \Return {``$b_{1}(x_{1}-t(1)) +\dots + b_{s}(x_{s}-t(s)) = 1$''}
\EndFunction
\end{algorithmic}
\end{algorithm}



%%
%%Then we factorize every constraint to get
%%a CSP instance $\Omega_{L}$ on domains $L_{1},\ldots,L_{n},Z_{p}$.
%%We know that the projection of
%%the solution set of $\Omega_{L}$ onto
%%the first $n$ variables is a full relation.
%%Therefore, the solution set can be defined by one linear equation with the variable $z$.
%%Hence, the solution set of


\begin{step}\label{nonLinkedStep}
Suppose $\Theta'$ is not linked. For each $i$ from $1$ to $k$
\begin{enumerate}
\item Check that for every $(a_{1},\ldots,a_{i})\in \mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{i}}$
there exist $(a_{i+1},\ldots,a_{k})\in \mathbb Z_{q_{i+1}}\times \dots \times \mathbb Z_{q_{k}}$ and  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item If yes, go to the next $i$.
\item If no, then find an equation
$c_{1}y_{1}+\dots+c_{i}y_{i}=c_{0}$ such that
for every $(a_{1},\ldots,a_{i})\in
\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{i}}$
satisfying $c_{1}a_{1}+\dots+c_{i}a_{i}=c_{0}$
there exist $(a_{i+1},\ldots,a_{k})\in \mathbb Z_{q_{i+1}}\times \dots \times \mathbb Z_{q_{k}}$ and  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item Add the equation $c_{1}y_{1}+\dots+c_{i}y_{i}=c_{0}$ to Eq.
\item Go to Step~\ref{AddingEquationCycle}.
\end{enumerate}
\end{step}

If $\Theta'$ is linked, then by Theorem~\ref{LinearStep} there exists a constraint
$((x_{i_1},\ldots,x_{i_s}),\rho)$ in $\Theta'$
and a subuniverse $\sigma$ of $\mathbf{D_{i_1}}\times\dots\times \mathbf{D_{i_s}}\times \mathbf{\mathbb Z_{p}}$
such that
the projection of $\sigma$ onto the first $s$ coordinates
is bigger than $\rho$ but
the projection of $\sigma\cap (D_{i_1}\times\dots\times D_{i_s}\times \{0\})$
onto the first $s$ coordinates is equal to $\rho$.
Then we add a new variable $z$ with domain $\mathbb Z_{p}$
and replace
$((x_{i_1},\ldots,x_{i_s}),\rho)$ by
$((x_{i_1},\ldots,x_{i_s},z),\sigma)$.
We denote the obtained instance by $\Upsilon$.
Let
$L$ be the set of all tuples $(a_{1},\ldots,a_{k},b)\in
\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}} \times \mathbb Z_{p}$
such that $\Upsilon$ has a solution with $z=b$ in $\phi(a_{1},\ldots,a_{k})$.
We know that the projection of $L$ onto
the first $n$ coordinates is a full relation.
Therefore $L$ is defined by one linear equation.
If this equation is $z = b$ for some $b\neq 0$, then
both $\Theta'$ and $\Theta$ have no solutions.
Otherwise, we put $z=0$ in this equation and get
an equation that describes all $(a_{1},\ldots,a_{k})$ such that
$\Theta'$ has a solution in $\phi(a_{1},\ldots,a_{k})$.
It remains to find this equation.

\begin{step}\label{LinkedStep}
Suppose $\Theta'$ is linked.
\begin{enumerate}
\item Find
an equation
$c_{1}y_{1}+\dots+c_{k}y_{k} = c_{0}$
such that
for every $(a_{1},\ldots,a_{k})\in
(\mathbb Z_{q_{1}}\times \dots \times \mathbb Z_{q_{k}})$
satisfying $c_{1}a_{1}+\dots+c_{k}a_{k}=c_{0}$
there exists  a solution of $\Theta'$
in $\phi(a_{1},\ldots,a_{k})$.
\item If the equation was not found then $\Theta$ has no solutions.
\item Add the equation $c_{1}a_{1}+\dots+c_{k}a_{k}=c_{0}$ to Eq.
\item Go to Step~\ref{AddingEquationCycle}.
\end{enumerate}
\end{step}




\begin{algorithm}
\begin{algorithmic}[1]
\Function{\FindEquationsForNonlinked}{$\Theta$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a linear system of equations $\phi$}
    \State{Let $\psi$ be a natural bijection from $\mathbb Z_{j_{1}}\times \dots \times \mathbb Z_{j_{s}}\to L_{1}\times\dots\times L_{n}$}   
    \State{$I := \{1\}$}     \Comment{$I$ is the set of independent variables}
    \State{$E := \varnothing$}     \Comment{We start with an empty set of equations}    
   \For{$j=1,2,\ldots,s$}
    \State{$e = \FindOneEquation(\Theta,\psi,I,\mbox{``Not linked"})$}     \Comment{Something about the equations}
    \If{$e = \mbox{``$0=0$"}$} 
        \State{$I := I\cup \{j\}$}
    \ElsIf{$e = \mbox{``$0=1$"}$}
        \Return{$\mbox{``No solution"}$}
    \Else
        \State{$E := E\cup e$}     \Comment{Add the equation we found}    
    \EndIf
    \EndFor
    \Return {$E$};
\EndFunction
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckTuple}{$\Theta,\phi,I,t,\type$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\Theta$, a solution of a linear system of equations $\phi$}
\If{$\type = \mbox{``Linked"}$}
    \If{$\Solve(\Reduce(\Theta,\phi(t))) = \mbox{``Solution"}$}
        \Return{true}
    \Else
        ~\Return{false}
    \EndIf
\Else
    \State{$R:=\{\alpha\in \mathbb Z_{j_{1}}\times \dots\times \mathbb Z_{j_{s}}\mid \proj_{I}(\alpha) = t\}$}    
    \Comment{We don't really calculate $R$}
    \For{$i=1,2,\ldots,n$}
        \State{$E_{i}:=\proj_{i}(\phi(R))$} \Comment{We calculate $E_{i}$}
    \EndFor
    \If{$\SolveNonlinked(\Reduce(\Theta,(E_{1},\dots,E_{n})) = \mbox{``Solution''}$}
        \Return true
    \Else 
        ~\Return false
    \EndIf
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

%            \State{$R := \{\alpha\in Z_{j_{1}}\times \dots \times \mathbb Z_{j_{s}}
%            \mid \forall i\in I \colon \proj_{I}(\alpha) = (0,0$}
%            \State{$D_{i} := \proj(\mbox{``No"}$}







%\SolvedNonlinked
%\Reduce +
%\CheckCycleConsistency
%\CheckIrreducibility
%\CheckWeakerInstance
%\SolveLinearSystem +
%\FactorizeInstance + 
%\WeakenConstraint
%\RemoveTriv +




==> exp.tex <==



\subsection{PC Subuniverse}\label{PCSubsection}

\begin{lem}\label{ReflexivePCRelations}
Suppose
$A$ is a PC algebra and 
$\rho\subseteq A^{n}$ is a relation containing all
the constant tuples $(a,\dots,a)$. 
Then $\rho$ can be represented as a conjunction of
binary relations of the form $x_i = x_j$.\end{lem}
\begin{proof}
All constant operations preserve $\rho$, 
and together with the constant operations 
the algebra $A$ generates all operations on the set $A$.
Then $\rho$ is preserved by all operations on $A$, 
and by Theorem ??? from \cite{lau}
$\rho$ can be represented
as a conjunction of
binary relations of the form $x_i = x_j$.
\end{proof}


\begin{lem}\label{FindCenter}
Suppose $\rho\subseteq A\times B$ is a subdirect relation
and
$A$ is a PC algebra. Then either
for every $c\in B$ there exists a unique $a\in A$ such that $(a,c)\in \rho$,
or there exists $c\in B$ such that $(a,c)\in \rho$ for every $a\in A$.
\end{lem}

\begin{proof}
Put
$\sigma_{l}(x_1,x_2,\ldots,x_{l}) = \exists y \;\rho(x_{1},y)
\wedge\dots\wedge \rho(x_{l},y).$
It is not hard to see that 
$\sigma_{l}$ contains all constant tuples.
Therefore, 
Lemma~\ref{ReflexivePCRelations} implies that $\sigma_{2}$ is either full, or the equality relation.

If $\sigma_{2}$ is the equality relation, then
for every $c\in B$ there exists a unique $a\in A$ such that $(a,c)\in \rho$.

Suppose $\sigma_2$ is full.
Then we consider the minimal $l$, 
if it exists, such that $\sigma_{l}$ is not full.
Since $\sigma_{l-1}$ is full, 
the relation $\sigma_{l}$ contains all tuples 
whose elements are not different.
Then 
Lemma~\ref{ReflexivePCRelations}
implies that $\sigma_{l}$ is a full 
relation, which means 
$\sigma_{l}$ is a full relation for every $l$.
Hence, for some $c$ we have $(a,c)\in \rho$ for every $a\in A$.
\end{proof}

The next two lemmas are easy to prove.

\begin{lem}
$A/\ConPC(A)$ has no nontrivial binary absorbing subuniverse or center.
\end{lem}

\begin{lem}
Suppose $B$ is a PC subuniverse of $A$, 
then 
$\{b/\ConPC(A)\mid b\in B\}$ is a PC 
subuniverse of 
$A/\ConPC(A)$.
\end{lem}

\begin{lem}\label{PCImpliesShort}
Suppose $\rho A\times B$ is a subdirect relation.
$A'$ is a PC subunivserse of $A$, 
there is no nontrivial binary absorbing subuniverse or center on $B$, and 
$B' = \proj_{1}((A'\times B)\cap\rho)$.
Then $B'$ is a PC subuniverse in $B$.
\end{lem}

\begin{proof}
Suppose 
$A' = E_{1}\cap\dots\cap E_{s}$, 
where each $E_{i}$ is an equivalence class of a PC congruence
$\sigma_{i}$ on $A$.
For every $i$ consider a relation 
$\rho_{i}\subseteq (A/\sigma_{i})\times B$, 
containing all pairs 
$(a/\sigma_{i},b)$ such that $(a,b)\in \rho$.
Since  the algebra $A/\sigma_{i}$ has non nontrivial binary absorbing subuniverse and 
$B$ has no nontrivial center, 
for every $b\in B$ there exists a unique 
element $E\in A/\sigma_{i}$
such that $(E,b)\in \rho_{i}$.
Put 
$\delta_{i}$ be the set of all tuples $(b_{1},b_{2})$
such that  

By Lemma~\ref{FindCenter}, i


\end{proof}



\begin{lem}\label{PCImpliesNew}
Suppose $\rho \subseteq A_{1}\times\dots\times A_{n}$ is a subdirect relation,
there is no nontrivial binary absorbing subuniverse or center on $A_{1}$, and 
$C = \proj_{1}((C_{1}\times\dots \times C_{n})\cap\rho)$,
where $C_{i}$ is a PC subuniverse in $A_{i}$ for every $i$.
Then $C$ is a PC subuniverse in $A_{1}$ or 
$C$ is empty.
\end{lem}
\begin{proof}
Let 
$R\subseteq (A_{1}\times\dots\times A_{n})\times A_{1}$,
be the set of all tuples
$((a_{1},\dots,a_{n}),a_{1})$
such that $(a_{1},\dots,a_{n})\in\rho$.
Since $\rho$ is subdirect, 
Lemma~\ref{} implies that 
$\rho' = (C_{1}\times\dots \times C_{n})\cap\rho)$ is a PC subuniverse of $\rho$.

Then Lemma~\ref{} implies that 
$C = \proj(R\cap (\rho'\times A_{1}))$ is a PC 
subuniverse of $A_{1}$.
\end{proof}



\begin{lem}\label{PCRelationsLem}
Suppose $\rho\subseteq A_1\times\dots \times A_{n}$ is a subdirect relation,
$A_{i}$ is a PC algebra for every $i\in\{2,\ldots,n\}$,
and there is no nontrivial 
binary absorbing subuniverse or nontrivial center on $A_{i}$ for every $i\in\{1,\ldots,n\}$.
Then $\rho$ can be represented as a conjunction of binary relations $\delta_{1},\ldots,\delta_{k}$ such that
$\ConOne(\delta_{l},j)$ is the equality relation whenever the domain of the $j$-th variable of $\delta_{l}$ is a PC algebra.
\end{lem}

This lemma 
says that 
the relation $\rho$ can be represented by 
constraints 
from the first coordinate to an $i$-th coordinate such that 
the $i$-th coordinate is uniquely determined by the first 
(also we can define the corresponding PC congruence on the first coordinate 
using this relation)
and by bijective binary constraints between pairs of coordinates
other than first.
Also it says that in a subdirect product of PC algebras without a nontrivial binary absorption or center (even $A_{1}$ is a PC algebra) we can choose some essential coordinates which can have any value, each other coordinate is uniquely determined by exactly one of them (in a bijective way).

\begin{proof}
We prove this lemma by induction on the 
arity of $\rho$. 
Assume that $\rho$ is not essential, then it can be represented as a conjunction of essential relations satisfying the same properties.
By the inductive assumption, each of them
can be represented as a conjunction of binary relations. It remains to join these binary relations to complete the proof for this case.


Assume that $\rho$ is essential.
The projection of $\rho$ onto any proper set of variables gives a relation of a smaller arity satisfying the same properties.
By the inductive assumption, the relation of a smaller arity can be represented as a conjunction of binary relations
$\delta_{1},\ldots,\delta_{k}$ such that
$\ConOne(\delta_{l},j)$ is the equality relation whenever the domain of the $j$-th variable of $\delta_{l}$ is a PC algebra.
In each relation 
$\delta_{i}$ 
one variable (let it be the $u$-th variable) is uniquely determined 
by another,
and therefore 
the relation 
$\rho$ can be represented as 
a conjunction of $\delta$ 
and the projection of 
$\rho$ onto all variables but $u$-th, 
which cannot happen
with an essential relation.
Therefore, 
each projection of $\rho$ onto any proper set of variables
is a full relation.

Let us consider the relation $\rho\subseteq (A_{1}\times\dots\times A_{n-1})\times A_{n}$ as a binary relation.
By Lemma~\ref{FindCenter} we have one of the following two situations.

Case 1: 
there exist $b_{1},\ldots,b_{n-1}$ such that $(b_{1},\ldots,b_{n-1},a)\in \rho$ for every $a\in A_{n}$.
We consider the maximal $s$ such that
$\rho(b_{1},\ldots,b_{s},x_{s+1},\ldots,x_{n})$ is not a full relation.
It is easy to see that $s\le n-2$ and $s$ exists.
By Lemma~\ref{GenBinAbToBinAb}, 
there is no 
nontrivial 
binary absorbing subuniverse 
on 
$A_{s+2}\times\dots\times A_{n}$,
then we get a nontrivial center $C$ on $A_{s+1}$
defined
by
$C = \{a_{s+1}\in A_{s+1}\mid \forall a_{s+2}\dots\forall a_{n} \colon
(b_{1},\ldots,b_{s},a_{s+1},a_{s+2},\ldots,a_{n})\in\rho\}$.


Case 2: for every $a_{1},\ldots,a_{n-1}$ there exists a unique $b$ such that
$(a_{1},\ldots,a_{n-1},b)\in \rho$.
If the relation $\rho$ is binary, then 
we already have the necessary condition.

Otherwise, we show in the same way that 
for any $(a_{1},a_{3},\ldots,a_{n})$
there exists a unique $b$ such that
$(a_{1},b,a_{3}\ldots,a_{n})\in\rho$.
Let us consider the relation 
$\zeta$ defined by
\begin{align*}\zeta(z_{1},z_{2},z_{3},z_{4}) =
\exists x_{1} \exists x_{2}\dots\exists x_{n-1} \exists x_{1}' \exists x_{2}'\;
&\rho(x_{1},x_{2},x_{3},\ldots,x_{n-1},z_{1})\wedge\\
\rho(x_{1},x_{2}',x_{3},\ldots,x_{n-1},z_{2})\wedge
&\rho(x_{1}',x_{2},x_{3},\ldots,x_{n-1},z_{3})\wedge
\rho(x_{1}',x_{2}',x_{3},\ldots,x_{n-1},z_{4}).
\end{align*}
Since 
any projection of $\rho$ onto any proper set of variables gives a full relation, 
any projection of 
$\zeta$ onto 3 variables is a full relation.
Since $\rho$ is subdirect, 
$\zeta$ contains all constant tuples
$(a,a,a,a)$, 
and by Lemma~\ref{ReflexivePCRelations}, 
$\zeta$ is a full relation.
Suppose $a\neq b$ and 
$(a,a,a,b)\in\zeta$
witnessed by 
$x_{1},\ldots,x_{n-1},x_{1}',x_{2}'$.
By the remark at the start 
of Case 2 we have 
$x_{2} = x_{2}'$ and 
therefore $a=b$. 
Contradiction.
\end{proof}

%It follows from Lemma~\ref{PCRelationsLem} that the %quotient of any algebra $\mathbf A$ without
%a center and binary absorption by $\ConPC(\mathbf A)$ is %a direct product of PC algebras.


\begin{conslem}\label{PCProperties}
Suppose $\sigma_{1},\ldots,\sigma_{k}$ 
are all PC congruences on $A$.
Put $A_{i} = A/\sigma_{i}$, 
and define 
$\psi:A\to A_{1}\times \dots\times A_{k}$
by $\psi(a) = (a/\sigma_{1},\dots,a/\sigma_{k})$. Then 
\begin{enumerate}
    \item $\psi$ is surjective, hence 
    $A/\PCCon(A)\cong A_{1}\times\dots\times A_{k}$.
    \item the PC subuniverses are the sets of the form 
    $\psi^{-1}(S)$, where $S\subseteq A_{1}\times \dots\times A_{k}$
    is a relation definable by unary constraints of the form 
    $x_{j} = a_{j}$.
    \item for each PC subuniverse $B$ of $A$ there is a congruence 
    $\theta$ of $A$ such that $B$ is an equivalence class of $\theta$ 
    and 
    $A/\theta$ is isomorphic to a product of PC algebras
    having no nontrivial binary absorbing subuniverse or center.
\end{enumerate}
\end{conslem}

\begin{proof}
First, notice that 
by Corollaries~\ref{AbsorptionQuotient} and 
\ref{CenterQuotient} there does not exist 
a nontrivial absorption or center on $A_{i}$ for any $i$.

Consider 
the image 
$\psi(A)$, which is a subdirect subuniverse 
of $A_{1}\times\dots\times A_{k}$.
By Lemma~\ref{PCRelationsLem},
this relation can be represented as a conjunction of binary relations whose one coordinate uniquely determines another (in a bijective way).
This means that congruences $\sigma_{i}$ corresponding to 
these coordinates should be equal, which contradicts the definition.
Then $\psi(A)$ is a full relation and $\psi$ is surjective.

The second item follows just from the definition of 
a PC subuniverse.

To prove the third item, just consider the intersection 
of all congruences whose equivalence classes we intersected to define
the PC subuniverse.
Then, in the same way as in the first item we prove 
the isomorphism.
\end{proof}
\begin{conslem}\label{PCImplies}
Suppose $\rho \subseteq A_{1}\times\dots\times A_{n}$ is a subdirect relation,
there is no nontrivial binary absorbing subuniverse or center on $A_{1}$, and 
$C = \proj_{1}((C_{1}\times\dots \times C_{n})\cap\rho)$,
where $C_{i}$ is a PC subuniverse in $A_{i}$ for every $i$.
Then $C$ is a PC subuniverse in $A_{1}$ or 
$C$ is empty.
\end{conslem}

\begin{proof}
By the previous corollary
for every $i$ we choose
PC algebras $A_{i,1},\dots,A_{i,k_{i}}$ 
and a mapping $\psi_{i}:A_{i}\to A_{i,1},\dots,A_{i,k_{i}}$
such that 
$A_{i}/\PCCon(A_{i})\cong A_{i,1}\times \dots\times A_{i,k_{i}}$.
%Again, notice that 
%by Corollaries~\ref{AbsorptionQuotient} and 
%\ref{CenterQuotient} these PC algebras have no
%a nontrivial absorption or center.
Define 
$\phi:A_{1}\times\dots\times A_{n}\to
A_{1}\times \prod_{i,j} A_{i,j}$ by 
$\phi(a_1,\dots,a_{n}) = (a_1,\psi_{1}(a_1),\ldots,\psi_{n}(a_n))$.
Let 
$\gamma = C_{1}\times\dots\times C_{n}$,
$\rho' = \phi(\rho)$, $\gamma'= \phi(\gamma)$.
We can check that 
$\proj_{1}(\rho\cap\gamma) = \proj_{1}(\rho'\cap\gamma')$, 
then it is sufficient to show that 
$\proj_{1}(\rho'\cap\gamma')$ is a PC subuniverse of 
$A_{1}$. 
Note that if $\proj_{1}(\rho'\cap\gamma')$ 
then we are done, thus we assume that it  is not empty.

Since $\rho'$ is subdirect, 
by Lemma~\ref{PCRelationsLem}
it can be represented 
by binary constraints from the first coordinate
to an $i$-th coordinate such that 
the $i$-th coordinate is uniquely determined by the first,
and by bijective binary constraints between pairs of coordinates
other than first.
$\gamma'$ can be represented by 
constraints of the form 
$x_{i,j} = a_{i,j}$ and 
canonical constraints 
saying that the $j$-th element of $\psi_{1}(x_{1})$ 
is equal to $x_{1,j}$.
To calculate 
$\proj_{1}(\rho'\cap \gamma')$ 
we join constraints of these two representations.
Let us explain how any constraint 
from $x_{1}$ to $x_{i,j}$ in this representation looks like.
There exists a congruence $\sigma$ on $A_{1}$ 
such that $A_{1}/\sigma$ is a PC algebra isomorphic to 
$A_{i,j}$, then the constraint  
assigns to all elements of each equivalence class of $\sigma$ 
the corresponding element of $A_{i,j}$.
All other constraints of this representations are 
of the form 
$x_{i,j} = a_{i,j}$
or bijective constraints between two coordinates.
This implies that 
$\proj_{1}(\rho'\cap\gamma')$ is an intersection of equivalence classes
of PC congruences, that is, $\proj_{1}(\rho'\cap\gamma')$ is a PC subuniverse.
\end{proof}
\begin{conslem}\label{PCLessThanThree}
Suppose
$\rho\subseteq A_{1}\times \dots \times A_{k}$ is a subdirect relation,
$k\ge 3$,
$C_{i}$ is a PC subuniverse in $A_{i}$,
and
there is no binary absorption or center on $A_{i}$ for every $i$.
There does not exist
a $(C_{1},\dots,C_{k})$-essential relation.
\end{conslem}

\begin{proof}
By Corollary~\ref{PCProperties}
for every $i$ we choose
PC algebras $A_{i,1},\dots,A_{i,k_{i}}$ 
and a mapping $\psi_{i}:A\to A_{i,1},\dots,A_{i,k_{i}}$
such that 
$A_{i}/\PCCon(A_{i})\cong A_{i,1}\times \dots\times A_{i,k_{i}}$.
By Corollaries~\ref{AbsorptionQuotient} and 
\ref{CenterQuotient} these PC algebras have no
a nontrivial absorption or center.
Define 
$\phi:A_{1}\times\dots\times A_{n}\to
\prod_{i,j} A_{i,j}$ by 
$\phi(a) = 
(\psi_{1}(a),\ldots,\psi_{n}(a))$.
Let 
$\gamma_{i} = C_{1}\times\dots\times
C_{i-1}\times A_{i}\times C_{i+1}\times\dots\times C_{n}$
for every $i$
and 
$\gamma = 
C_{1}\times\dots\times C_{n}$.
Put 
$\rho' = \phi(\rho)$, $\gamma'= \phi(\gamma)$,
$\gamma_{i}'= \phi(\gamma_{i})$ for every $i$.

Since $\rho'$ is subdirect, by Lemma~\ref{PCRelationsLem}
$\rho'$ can be represented 
by bijective binary constraints between pairs.
By Corollary~\ref{PCProperties}
$\gamma'$ can be represented by 
constraints of the form 
$x_{i,j} = a_{i,j}$.
If $\rho\cap\gamma=\varnothing$, 
then 
$\rho'\cap\gamma'=\varnothing$, 
which can only happen 
if two unary constraints defining 
$\gamma'$ assign contradictory values to 
variables with respect to the binary 
constraints defining $\rho'$.
Since $k\ge 3$, we can choose
$l$ 
such that 
$\gamma_{l}'$ includes the two contradictory
unary constraints.
Then $\rho'\cap \gamma_{l}'=\varnothing$
and $\rho\cap \gamma_{l}=\varnothing$, 
which gives a contradiction.
\end{proof}


\begin{lem}\label{BiggerThanPC}
Suppose 
$\sigma\supseteq \sigma_{1}\cap \dots\cap \sigma_{n}$,
where $\sigma_{1},\dots,\sigma_{n}$ are PC congruence on $D$ 
and $\sigma$ is a congruence on $D$.
Then there exists $I\subseteq \{1,2,\dots,n\}$
such that 
$\sigma = \bigcap_{i\in I}\sigma_{i}$.
\end{lem}
\begin{proof}
Consider a $2n$-ary relation 
$R\subseteq D/\sigma_{1}\times\dots\times D/\sigma_{n}
\times D/\sigma_{1}\times\dots\times D/\sigma_{n}$
consisting of all 
tuples 
$(a/\sigma_{1},\dots,a/\sigma_{n},b/\sigma_{1},\dots,b/\sigma_{n})$, where 
$(a,b)\in \sigma$.
By Lemma~\ref{PCRelationsLem}, 
$R$ can be represented as a conjunction of binary 
relations.
Since 
$(a/\sigma_{1},\dots,a/\sigma_{n},a/\sigma_{1},\dots,a/\sigma_{n})\in R$ for every $a\in D$, 
we conclude that all these binary relations are equalities.
This implies that 
$\sigma = \bigcap_{i\in I}\sigma_{i}$
for some $I\subseteq \{1,2,\dots,n\}$.
\end{proof}

\begin{remark}\label{PCFactorizationRemark}
The phrase 
``We factorize variables
$y_{1},\ldots,y_{n}$
of a relation $\rho(x_{1},\ldots,x_{n},y_{1},\dots,y_{s})$ by $\ConPC(y_{i}), i=1,2,\dots,s$
and replace them by PC variables''
means the following.
For each variable $y_{i}$,
by Corollary~\ref{PCProperties}
there exist PC algebras
$A_{i,1},\ldots,A_{i,k_{i}}$ 
and 
an isomorphism $\psi_{i}: D_{y_{i}}/\PCCon(D_{y_{i}})\cong A_{i,1}\times\dots\times A_{i,k_{i}}$.
Note that 
there is no nontrivial absorption or center in each $A_{i,j}$  by Corollaries~\ref{AbsorptionQuotient},
\ref{CenterQuotient}.
We replace each $y_{i}$ with PC variables
$u_{i,1},\dots,u_{i,k_{i}}$
with domains $A_{i,1},\dots,A_{i,k_{i}}$
and define 
$\delta\subseteq
D_{x_{1}}\times \dots\times D_{x_{n}}\times \prod_{i,j} A_{i,j}$ by
%$$\delta(x_{1},\ldots,x_{n}, (u_{i,j})_{i,j}) = 
\begin{align*}\{(a_{1},\ldots,a_{n}, (b_{i,j})_{i,j})
\mid 
\exists c_{1},\ldots,c_{s}\colon
(a_{1},\ldots,a_{n},c_{1},\ldots,c_{s})\in&\rho
\wedge \\
&\psi_{i}(c_{i}/\ConPC(D_{y_{i}})) = 
(b_{i,1},\dots,b_{i,k_{i}})
\}
\end{align*}
\end{remark}


\begin{lem}\label{NoAbsCenterInPCAlgebra}
For every $D$ the algebra $D/\ConPC(D)$
has no nontrivial binary absorbing subuniverse 
or center.
\end{lem}
\begin{proof}
Assume the converse.
By Corollary~\ref{PCProperties},
$A/\PCCon(A)\cong A_{1}\times\dots\times A_{k}$, 
where $A_{i}$ is a PC algebra without binary absorption or center.
By Lemmas~\ref{GenBinAbToBinAb} and \ref{GenCenterToCenter},
there exists a nontrivial binary absorption or a center
on $A_{i}$ for some $i$, which contradicts our assumptions.
\end{proof}

\begin{lem}\label{PCCongruenceOnProduct}
Suppose 
$\sigma$ is a PC congruence on $A_{1}\times A_{2}$, 
no binary absorption or center on $A_{1}$ and $A_{2}$.
Then there exist $i\in\{1,2\}$ and a PC congruence $\sigma_{i}$ on $A_{i}$ 
such that 
$\sigma = 
\{(\alpha,\beta)\mid (\proj_{i}(\alpha), \proj_{i}(\beta))\in\sigma_{i}\}$.
%$\sigma = \{((a_{1,1},a_{1,2}),(a_{2,1},a_{2,2}))\mid 
%(a_{1,i},a_{2,i})\in\sigma_{i}\}$.
\end{lem}
\begin{proof}
First, consider the 
binary relation 
$S\subseteq A_{1}\times (A_{1}\times A_{2})/\sigma$ 
consisting of all pairs 
$(a_1,(a_1,a_2)/\sigma)$, where $a_1\in A_{1}$, $a_{2}\in A_{2}$.
Since there is no binary absorption or center on $A_{1}$,  Lemma~\ref{PCRelationsLem} implies that either 
$S$ is a full relation, or 
$\ConOne(S,2)$ is the equality relation.
In the later case
the congruence $\sigma$ depends only on the first coordinate, 
that is, 
there exists a PC congruence 
$\sigma_{1}$ on $A_{1}$ 
such that 
$\sigma = 
\{(\alpha,\beta)\mid (\proj_{1}(\alpha), \proj_{1}(\beta))\in\sigma_{1}\}$,
%$\sigma = 
%\{((a_{1,1},a_{1,2}),(a_{2,1},a_{2,2}))\mid 
%(a_{1,1},a_{2,1})\in\sigma_{1}\}$, 
which completes this case.

Thus, we assume that $S$ is a full relation and 
for every $a_1\in A_1$ and every equivalence class
$E$ of $\sigma$ there exists $a_{2}\in A_{2}$ such 
that $(a_{1},a_{2})\in E$.
In the same way, we assume that 
for every $a_2\in A_2$ and every equivalence class
$E$ of $\sigma$ there exists $a_{1}\in A_{1}$ such 
that $(a_{1},a_{2})\in E$.

Choose an element $c_1\in A_{1}$.
By $\sigma_{2}$ we denote the congruence 
$\{(a_{2},a_{2}')\mid 
((c_{1},a_{2}),(c_{1},a_{2}'))\in\sigma\}$.
As it follows from the above assumptions, 
$A_{2}/\sigma_{2}\cong (A_{1}\times A_{2})/\sigma$.
Consider a ternary relation
$\rho\subseteq A_{1}\times (A_{1}\times A_{2})/\sigma\times 
A_{2}/\sigma_{2}$ consisting of 
all the tuples 
$(a_1,(a_{1},a_{2})/\sigma,a_{2}/\sigma_{2})$,
where $a_{1}\in A_{1}$ and $a_{2}\in A_{2}$.
As we already know, the projection of $\rho$ onto any two coordinates 
is a full relation. Then Lemma~\ref{PCRelationsLem}
implies that $\rho$ is a full relation, 
which contradicts the fact that 
$(c_{1},(c_{1},a_{2})/\sigma,b_{2}/\sigma_{2})\notin\rho$ 
if $(a_{2},b_{2})\notin \sigma_{2}$.
This completes the proof.
\end{proof}

\begin{conslem}\label{PCCongruenceOnProductGen}
Suppose 
$\sigma$ is a PC congruence on $A_{1}\times A_{2}\times\dots\times A_{n}$, 
no binary absorption or center on $A_{i}$ for every $i$.
Then there exist $i\in\{1,2,\dots,n\}$ and a PC congruence $\sigma_{i}$ on $A_{i}$ 
such that 
$\sigma = 
\{(\alpha,\beta)\mid (\proj_{i}(\alpha), \proj_{i}(\beta))\in\sigma_{i}\}$.
\end{conslem}

\begin{proof}
We prove by induction on $n$.
For $n=2$ it follows from Lemma~\ref{PCCongruenceOnProduct}.
By Lemmas~\ref{GenBinAbToBinAb}, \ref{GenCenterToCenter},
there is no binary absorption or center on 
$A_{2}\times\dots\times A_{n}$.
We apply 
Lemma~\ref{PCCongruenceOnProduct} to 
$A_{1}\times(A_{2}\times\dots\times A_{n})$ 
to get a PC congruence on 
$A_{1}$ or on $A_{2}\times\dots\times A_{n}$.
In the later case we apply the inductive assumption to complete the proof.
\end{proof}

\begin{lem}\label{PCSubuniverseOnProduct}
Suppose 
$B$ is a PC subuniverse on 
$A_{1}\times\dots\times A_{n}$, 
there is no binary absorption or center on $A_{i}$
for every $i$.
Then there exists 
a PC subuniverse 
$B_{i}$ on $A_{i}$ for every $i$ such that 
$B = B_{1}\times\dots\times B_{n}$.
\end{lem}
\begin{proof}
Assume that 
$B=E_{1}\cap\dots\cap E_{t}$, 
where $E_{i}$ is an equivalence class of a PC congruence $\sigma_{i}$ on $A_{1}\times\dots\times A_{n}$ for every $i$.
By Corollary~\ref{PCCongruenceOnProductGen},
for every $i$ there exists 
$s_{i}$ and a congruence $\sigma_{i}'$ on $A_{s_{i}}$ such that 
$\sigma_{i} = \{(\alpha,\beta)\mid (\proj_{s_{i}}(\alpha), \proj_{s_{i}}(\beta))\in\sigma_{i}'\}$.
Then there exists an equivalence class $E_{i}'$ of $\sigma_{i}'$
such that 
$E_{i} = 
A_{1}\times\dots\times A_{s_{i}-1}\times 
E_{i}'\times A_{s_{i}+1}\times\dots\times A_{n}$.
Hence, the intersection $E_{1}\cap\dots\cap E_{t}$ 
is equal to $B_{1}\times\dots\times B_{n}$
for PC subuniverses $B_{1},\dots,B_{n}$. 
\end{proof}


\begin{lem}\label{CenterProvidesBinaryAbsorptionForPC}
Suppose
$\rho\subseteq A\times B$ is a subdirect relation,
$A$ is a PC algebra without a nontrivial center or binary absorbing subuniverse, and 
$C = \{b\in B\mid \forall a\in A\colon (a,b)\in \rho\}$.
Then $C$ binary absorbs $B$.
\end{lem}

\begin{proof}
Suppose $A = \{a_{1},\ldots,a_{k}\}$.
Let us consider the matrix $M$
whose rows are the tuples
$(\underbrace{a,a,\ldots,a}_{k+1},b,a_{1},\ldots,a_{k})$
and $(b,a_{1},\ldots,a_{k},\underbrace{a,a,\ldots,a}_{k+1})$
for all $a,b\in A$.
The $2k+2$ columns of this matrix we denote by
$\alpha_{1},\ldots,\alpha_{2k+2}$.
By $\beta$ we denote the tuple of length $2k^2$
such that the $i$-th element of $\beta$ equals $b$ from the corresponding row.
By Lemma~\ref{PCRelationsLem},
%By $\delta$ we denote the relation
the relation
generated by $\alpha_{1},\ldots,\alpha_{2k+2}$
is a full relation.
Hence, there exists
a term operation $f$
such that
$f(\alpha_{1},\ldots,\alpha_{2k+2})=\beta$.
Let us show that $C$ absorbs $B$ with the term operation defined by
$h(x,y)=f(\underbrace{x,\ldots,x}_{k+1},y,\ldots,y)$.
Suppose $d\in B$, $c\in C$.
Assume that $h(d,c)=e\notin C$.
Choose elements $a,a'\in A$ such that
$(a,e)\notin\rho$ and
$(a',d)\in\rho$.
Consider the row
$(a',\ldots,a',a,a_{1},\ldots,a_{k})$ from the matrix.
We know that
$f$ returns $a$ on this tuple
and
$f(\underbrace{d,\ldots,d}_{k+1},c,\ldots,c) = e$, which contradicts the fact that
$f$ preserves $\rho$.

In the same way we prove that $h(c,d)\in C$
for every $d\in B$, $c\in C$.
\end{proof}




\begin{lem}\label{IdentificationDoesNotReducePC}
Suppose
$\rho\subseteq A\times B\times B$ is a subdirect relation,
$A$ is a PC algebra without a center and a binary absorption,
for every $b\in B$ there exists $a\in A$ such that
$(a,b,b)\in \rho$.
Then for every $a\in A$ there exists $b\in B$ such that
$(a,b,b)\in\rho$.
\end{lem}
\begin{proof}
We prove the lemma by induction on the size of $B$.
%For $l=2,3,\ldots$
%put
%$\sigma_{l}(x_{1},\ldots,x_{l}) =
%\exists y_{2}\exists y_{3}\; \rho(x_{1},y_{2},y_{3})\wedge\dots
%\wedge \rho(x_{l},y_{2},y_{3})$.

By Lemma~\ref{FindCenter}, only two situations are possible: either
there exists $c_{1},c_{2}\in B$ such that
$(a,c_{1},c_{2})\in \rho$ for every $a\in A$,
or
for all $(b_{1},b_{2})\in \proj_{2,3}(\rho)$ there exists a unique $a\in A$
such that $(a,b_{1},b_{2})\in \rho$.
Consider the first case.
Put $D = \{(b,c)\mid \forall a\in A\colon (a,b,c)\in\rho\}$.
By Lemma~\ref{CenterProvidesBinaryAbsorptionForPC}, $D$ is a binary absorbing subuniverse in the projection
of $\rho$ onto the last two variables.
By Lemma~\ref{AbsorbingEquality}, there exists $(b,b)\in D$. This completes this case.

Consider the second case.
Let $\delta_{1}$ be the projection of $\rho$ onto the first two variables.
By Lemma~\ref{FindCenter} we have one of two situations.
Assume that for every $b\in B$ there exists a unique $a$ such that
$(a,b)\in\delta_{1}$. Then we can check that
if $(a,b,b')\in\rho$ then $(a,b,b)\in\rho$, which completes this case.
%Then for every $a\in A$ we have $b$there exists a unique
%the statement can be easily checked.
Otherwise, there exists an element $b$ such that $(a,b)\in\delta_{1}$ for every $a\in A$.
Consider the relation
$\delta_{2}(x,y_{2}) = \rho(x,b,y_{2})$.
If $\proj_{2}(\delta_{2})\neq B$, then we restrict the last two variables of $\rho$ to $\proj_{2}(\delta_{2})$
and apply the inductive assumption.
Assume that $\proj_{2}(\delta_{2}) = B$.
By the definition of the second case %with Lemma~\ref{FindCenter}
we know that
for every $c\in B$ there exists a unique $a$ such that
$(a,c)\in\delta_{2}$.
Then $\sigma=\ConOne(\delta_2,2)$ 
is a proper congruence such that
$B/\sigma$ is a PC algebra.
%Then there exists a congruence $\sigma$ on $B$ such that $B/\sigma$ is a PC algebra.
If $\sigma$ is the equality relation, then $B$ is a PC algebra without center and binary absorption.
Then the statement follows from Lemma~\ref{PCRelationsLem}.
% hence
% the relation defined by $\rho(x,y,y)$ is subdirect.

If $\sigma$ is not the equality relation, then
we consider the relation $\rho'$ obtained from $\rho$ by factorization of the last two variables by $\sigma$.
By the inductive assumption for any $a\in A$ there exists $E\in B/\sigma$ such that
$(a,E,E)\in\rho'$.
By Lemma~\ref{FindCenter}, we have one of the following situations.
Case 1. There exists $E\in B/\sigma$ such that
for every $a\in A$ we have $(a,E,E)\in\rho'$.
Then we restrict the last two variables of $\rho$ to $E$ and apply the inductive assumption.
Case 2. For every $E\in B/\sigma$ there exists a unique $a\in A$
such that $(a,E,E)\in\rho'$.
In this case for any $a\in A$ we
choose $E$ such that $(a,E,E) \in \rho'$.
By the uniqueness of $a$ we have
$(a,b,b)\in \rho$ for any $b\in E$, which completes the proof.
\end{proof}

